Are Smart Home Devices Abandoning IPV Victims?

Smart home devices have brought us many benefits such as advanced security, convenience, and entertainment. However, these devices also have made unintended consequences like giving ultimate power for devices' owners over their intimate partners in the same household which might lead to tech-facilitated domestic abuse (tech-abuse) as recent research has shown. In this paper, we systematize findings on tech-abuse in smart homes. We show that domestic abuse and Intimate Partner Violence (IPV) in smart homes is more effective and less risky for abusers. Victims find it more harmful and more challenging to protect themselves from. We articulate a comprehensive analysis of all the phases of abuse in smart homes and categorize risks and needs in each phase. Technical analysis of current smart home technologies is conducted to shed light upon their limitations. We also summarize recent recommendations to combat tech-abuse in smart homes and focus on their potentials and shortcomings. Unsurprisingly, we find that many recommendations conflict with each other due to a lack of understanding of phases of abuse in smart homes. Desirable properties to design abuse-resistant smart home devices are proposed for all the phases of abuse. The research community benefits from our analysis and recommendations to move forward with a focus on filling the blind spots of existing smart home devices' safety measures and building appropriate safety measures that consider tech-abuse threats in smart homes.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> Tech-abuse_SmartHomes_Draft 2-3/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> Tech-abuse_SmartHomes_Draft 2-3/TexFiles/Acquiring.tex <==
This phase includes purchasing, setting up, and sharing access to smart home devices.
The research community has paid little attention to issues that occur during this phase even though the risk of imbalance in control starts here~\cite{power_Imbalance_Study,European_Cybersecurity_report_imbalanceControlProblem}. 
In a trusting environment, users share passwords to their devices or accounts with their partners~\cite{SmartHome_Abuse_Category_2_paper4}.
This is not an issue unless one partner starts to exploit the established trust.

Parkin et al. have considered a configuration phase in their work \cite{SmartHome_Abuse_Category_2_paper3}. 
However, we believe that the risk exists even before configuring the smart home device.
If users (potential victims) of smart home devices understand accurately what the capabilities of the devices are and what kind of control they offer, they may change their device purchase decision, as changes are easier to make before the purchase~\cite{PurchaseChange}. 
Given the fact that changing behaviors before acquiring the device is possible, we need to consider adding this phase as a crucial component of the abuse phases. 
If the research community puts effort to raise awareness of the devices' susceptibility to exploitation, consumers can make more educated choices. 
This will put pressure on vendors to pay attention to issues in SHOT, and will in turn motivate them to make their devices abuse-resistant.

Recently, a few organizations have attempted to score IoT devices based on their security, privacy, and safety measures~\cite{digital_Standard}. 
The Digital Standards project is run and maintained by the Consumer Report~\cite{consumerReport}. 
The goal is to build standards for IoT devices to help consumers choose the best options for them.
One criterion proposed by the Digital Standards is called ``personal safety.'' It accounts for the measures taken by smart home vendors to mitigate or respond to domestic abuse.
Unfortunately, the corresponding fields on the standard are not filled yet due to a lack of research focus on the matter.
Emami-Naeini et al. have also considered adding a personal safety label. However, more research needs to be conducted to come up with metrics to evaluate devices' capabilities regarding personal safety~\cite{Security_lables}.
We believe that our framework will help define future metrics by showing the different phases of abuse in SHOT and the corresponding device requirements for abuse-resistance. 
%The importance of showing real capabilities is discussed in this article~\cite{bcs_capabilities_importanace}. 

% Metrics to evaluate safety features in smart home devices need to account for the ability of abusers to abuse, hide their abuse, and destroy evidence of abuse. Metrics for victims can be: ability to have equal access to shared devices, ability to recognize abuse, ability to record abuse, and ability to revoke access. Metrics for support services: ability to have guidelines on how to help victims, ability to intervene, ability to . For vendors, following standards, providing guidelines, and implementing research recommendations

The goals in this phase are to limit abusers' excessive control power, educate victims on safety specifications of smart home devices, and assist support services.
First, the research community has proposed a few ways to prevent owners of smart home devices from gaining excessive control power over other users in the same household. 
Device vendors can deploy a setup process that involves other users such as asking the main user to answer whether there are other people living in the same house~\cite{SmartHome_Abuse_Category_2_paper1,power_Imbalance_Study}. 
This also calls for understanding the different levels of technical backgrounds among users. 
One limitation to this approach is that it relies on the honesty of owners to disclose such information, which can be challenging as device owners may pose a threat to the other users in an IPV setting. 
Future research needs to focus on how to enhance the setup process without fully relying on owners' disclosures. 
Second, empowering victims of IPV can be done by providing safety labels on smart home devices~\cite{digital_Standard,Security_lables}. %by making support resources reachable through smart home devices and 

Last, support services' goals consist of providing help to victims and holding abusers accountable. These services include front liners, law enforcement, and legal experts. 
Lopez-Neira et al. show that front liners in support organizations suffer from a lack of expertise to deal with SHOT~\cite{SmartHome_Abuse_Category_1_paper1}. 
The authors offer several recommendations such as involving cybersecurity experts to help make safety plans for victims along with front liners at support services.
In Section \ref{ourProposals}, we discuss solutions for current smart home devices. %in more detail. 
We also lay out the desired properties for each phase of the SHOT framework, including the acquiring and recognizing phases.
%\begin{itemize}
%    \item This phase is not in traditional domestic abuse
%    \item The reason why we created this phase is the importance of it as we can fix the authentication and awareness of device capabilities here
%    \item What is literature? 
%    \begin{itemize}
%        \item is it empowering abusers, victims or assisting support? 
%    \end{itemize}
%    \item Solutions proposed? Security labels should include safety labels or abuse-resistant fields.
%    \item Limitations?
%    \item Moving forward...
%    \begin{itemize}
%        \item How to limit abusers' power
%        \item How to empower victims
%        \item How to assist support services (law enforcement , legal, and charities)
 %   \end{itemize}
%\end{itemize}


\iffalse
This phase includes purchasing, setting up, and sharing access to smart home devices.
%The research community has paid little focus on issues that happen in this phase even though the risk of imbalance in control starts here~\cite{power_Imbalance_Study,European_Cybersecurity_report_imbalanceControlProblem}. 
The research community has paid little attention to issues that occur during this phase even though the risk of imbalance in control starts here~\cite{power_Imbalance_Study,European_Cybersecurity_report_imbalanceControlProblem}.
In a trusting environment, users share passwords to their devices or accounts with their partners~\cite{SmartHome_Abuse_Category_2_paper4}.
This is not an issue unless one partner starts to exploit the established trust.

Parkin et al. have considered a configuration phase in their work \cite{SmartHome_Abuse_Category_2_paper3}. 
However, we believe that the risk exists even before configuring the smart home device.
%If users (potential victims) of smart home devices understand accurately what the capabilities of the devices are and what kind of control they offer, users might change their minds since changes are easier to make before the purchase~\cite{PurchaseChange}. 
If users (potential victims) of smart home devices understand accurately what the capabilities of the devices are and what kind of control they offer, they may change their device purchase decision, as changes are easier to make before the purchase~\cite{PurchaseChange}. 
Given the fact that changing behaviors before acquiring the device is possible, we need to consider adding this phase as a crucial component of the abuse phases.
%Given the fact that changing behaviors before acquiring the device is possible makes us consider adding this phase as a crucial component in the abuse phases. 
If the research community puts effort to raise awareness of the devices' susceptibility to exploitation, consumers  can make more educated choices.
This will put pressure on vendors to pay attention to issues in SHOT, and will in turn motivate them to make their devices abuse-resistant.
% Above is Malek's edit, below first draft..
%If effort by the research community is put to raise awareness of unsafe devices that their capabilities could be exploited easily without any countermeasures, consumers are more likely to consider finding other alternatives. 
%This will put pressure on vendors to pay attention to issues in SHOT which might also motivate them to gain competitive advantages by considering making their devices abuse-resistant.

%Recently, a few organizations have attempted to give scores to IoT devices based on their security, privacy, and safety measures~\cite{digital_Standard}. 
Recently, a few organizations have attempted to score IoT devices based on their security, privacy, and safety measures~\cite{digital_Standard}.
The Digital Standards project is run and maintained by the Consumer Report~\cite{consumerReport}. 
The goal is to build standards for IoT devices to help consumers choose the best options for them.
One criterion proposed by the Digital Standards is called "personal safety." It accounts for the measures taken by smart home vendors to mitigate or respond to domestic abuse.
%One criterion that was proposed by the Digital Standards is called personal safety which accounts for the measures taken by smart home vendors to mitigate or respond to domestic abuse.
Unfortunately, the corresponding fields on the standard are not filled yet due to a lack of research focus on the matter.
Emami-Naeini et al. have also considered adding a personal safety label. However, more research needs to be conducted to come up with metrics to evaluate devices' capabilities regarding personal safety~\cite{Security_lables}.
We believe that our framework will help define future metrics by showing the different phases of abuse in SHOT and the corresponding device requirements for abuse-resistance. 
%Emami-Naeini et al. have also considered adding a personal safety label. However, more research needs to be conducted to come up with metrics that can be taken to evaluate devices' capabilities regarding personal safety~\cite{Security_lables}.
%We believe that our framework will help future metrics by showing the different phases of abuse in SHOT and their corresponding needs to be abuse-resistant. 
%The importance of showing real capabilities is discussed in this article~\cite{bcs_capabilities_importanace}. 

% Metrics to evaluate safety features in smart home devices need to account for the ability of abusers to abuse, hide their abuse, and destroy evidence of abuse. Metrics for victims can be: ability to have equal access to shared devices, ability to recognize abuse, ability to record abuse, and ability to revoke access. Metrics for support services: ability to have guidelines on how to help victims, ability to intervene, ability to . For vendors, following standards, providing guidelines, and implementing research recommendations

The goals in this phase are to limit abusers' excessive control power, educate victims on safety specifications of smart home devices, and assist support services.
First, the research community has proposed a few ways to prevent owners of smart home devices from gaining excessive control power over other users in the same household. 
Device vendors can deploy a setup process that involves other users such as asking the main user to answer whether there are other people living in the same house~\cite{SmartHome_Abuse_Category_2_paper1,power_Imbalance_Study}. 
This also calls for understanding the different levels of technical backgrounds among users. 
One limitation to this approach is that it relies on the honesty of owners to disclose such information, which can be challenging as device owners may pose a threat to the other users in an IPV setting. 
Future research needs to focus on how to enhance the setup process without fully relying on owners' disclosures.
Second, empowering victims of IPV can be done by providing safety labels on smart home devices~\cite{digital_Standard,Security_lables}. 
Last, support services' goals consist of providing help to victims and holding abusers accountable. These services include front liners, law enforcement, and legal experts.
Lopez-Neira et al. show that front liners in support organizations suffer from a lack of expertise to deal with SHOT~\cite{SmartHome_Abuse_Category_1_paper1}. 
The authors offered several recommendations such as involving cybersecurity experts to help make safety plans for victims along with front liners at support services.
In Section \ref{ourProposals}, we discuss solutions for current smart home devices in more detail. We also lay out the desired properties for each phase of the SHOT framework, including the acquiring and recognizing phases.
%\begin{itemize}
%    \item This phase is not in traditional domestic abuse
%    \item The reason why we created this phase is the importance of it as we can fix the authentication and awareness of device capabilities here
%    \item What is literature? 
%    \begin{itemize}
%        \item is it empowering abusers, victims or assisting support? 
%    \end{itemize}
%    \item Solutions proposed? Security labels should include safety labels or abuse-resistant fields.
%    \item Limitations?
%    \item Moving forward...
%    \begin{itemize}
%        \item How to limit abusers' power
%        \item How to empower victims
%        \item How to assist support services (law enforcement , legal, and charities)
 %   \end{itemize}
%\end{itemize}
\fi

==> Tech-abuse_SmartHomes_Draft 2-3/TexFiles/Acting.tex <==
This phase is not unique to tech-abuse in smart homes. %SHTA
Traditional methods of abuse and tech-abuse have considered this phase of abuse. 
Various legislative bodies and civil rights groups have fought to stop and prevent traditional abuse, and to hold abusers accountable by passing laws, pushing standards, and providing shelter resources. 
For instance, the Colorado state penalizes stalkers by prison sentences up to 10 years~\cite{colorado_law_stalking}. 
These strict laws may deter stalkers in traditional abuse cases.
However, building a legal case with evidence in tech-abuse can be challenging as abusers can find alternative ways to launch their abusive actions~\cite{NY_Times_Tech_Abuse}. 
Recent research has created new tools for victims of IPV to stop their abusers from having access to their phones~\cite{tech-abuse-helpVictims_1,tech-abuse-helpVictims_2}.
Even though the literature has not fully remedied tech-abuse using smartphones and personal computers, adequate resources have been developed for victims~\cite{Tech-abuse-smartphones-computers}.


\iffalse
This phase is not unique to tech-abuse in smart homes. %SHTA
Traditional methods of abuse and tech-abuse have considered this phase of abuse. 
The Legislature and research community have fought to stop, prevent traditional abuse, and hold abusers accountable by passing laws, pushing standards, and providing shelter resources. 
For instance, the Colorado state penalizes stalkers by prison sentences up to 10 years~\cite{colorado_law_stalking}. 
These strict laws might be effective to stop stalkers in traditional abuse.
However, building a legal case with evidence in tech-abuse can be challenging as abusers might find alternative ways to launch their abusive actions~\cite{NY_Times_Tech_Abuse}.
Recent research has created new tools for victims of IPV to stop their abusers from having access to their phones~\cite{tech-abuse-helpVictims_1,tech-abuse-helpVictims_2}.
Even though the literature has not fully remedied tech-abuse using smartphones and personal computers, adequate resources have been developed for victims~\cite{Tech-abuse-smartphones-computers}.
\fi

Compared to the previous approaches of abuse, empowering IPV victims using smart home devices with tools and resources has been limited. 
Some research projects aim to raise awareness and provide proper tools directly to the victims~\cite{SmartHome_Abuse_Category_2_paper1,SmartHome_Abuse_Category_2_paper2,SmartHome_Abuse_Category_2_paper3,SmartHome_Abuse_Category_2_paper4}. 
For example, Parkin et al. analyze two popular smart home devices: \textit{Google Home} and \textit{Amazon Alexa} for their usability in IPV. They find that remodeling the definition of usability in smart home devices is needed to meet the expectations of different entities involved in IPV~\cite{SmartHome_Abuse_Category_2_paper3}.
Others aim to facilitate support services for the victims through local organizations and law enforcement~\cite{SmartHome_Abuse_Category_1_paper1,SmartHome_Abuse_Category_2_paper4,SmartHome_Abuse_Category_3_paper1}.
For instance, authors in~\cite{SmartHome_Abuse_Category_1_paper1} recommend continuously training support services on emerging technologies so that they are well-prepared when fighting SHOT.


%Compared to the previous approaches of abuse, empowering IPV victims using smart home devices with tools and resources has been limited. 
%It makes sense as the smart home technologies are relatively new and challenges arise along the way.
%There have been some efforts by the research community to make resources for victims of IPV in smart homes. Some projects aim to raise awareness and provide proper tools directly to the victims~\cite{SmartHome_Abuse_Category_2_paper1,SmartHome_Abuse_Category_2_paper2,SmartHome_Abuse_Category_2_paper3,SmartHome_Abuse_Category_2_paper4}. 
%For example, Parkin et al. analyze two popular smart home devices: \textit{Google Home} and \textit{Amazon Alexa} for their usability in IPV and find that remodeling the definition of usability in smart home devices is needed to meet the expectations of different entities involved in IPV~\cite{SmartHome_Abuse_Category_2_paper3}.
%Others aim to facilitate support services for the victims through local organizations and law enforcement~\cite{SmartHome_Abuse_Category_1_paper1,SmartHome_Abuse_Category_2_paper4,SmartHome_Abuse_Category_3_paper1}.
%For instance, authors in~\cite{SmartHome_Abuse_Category_1_paper1} recommend constantly training support services with new emerging technologies to be equipped in fighting SHOT.

It is worth noting that smart home devices empower abusers by default. 
The work in~\cite{SmartHome_Abuse_Category_1_paper1,SmartHome_Abuse_Category_1_paper2,NDVH_abuse_signs} demonstrates that through interviews and workshop involving victims and support services. %~\cite{NDVH_abuse_signs}. 
In Section \ref{technical_causes}, we discuss the technical factors that empower abusers over victims in IPV.

One goal of this phase is to assist victims in gathering evidence, hiding their tracks for reaching out to support services, and building a legal case to escape safely. 
%After abuse is identified, victims aim to take actions like planning to confront abusers, look for help, and escape. 
Freed et al. show how dangerous this phase can be when victims start to take actions as abusers will escalate their aggressiveness~\cite{SmartHome_Abuse_Category_2_paper4}. 

The other goal is to mediate the help provided by support services to the victim such as facilitating a safe escape plan where abusers should not notice anything.
Islam et al. developed a system that recognizes abuse from the spoken language of victims using Natural Language Processing (NLP) tools~\cite{homeGuard_abuse_recognize_seekHelp}. 
It then evaluates the abuse and reaches out to the nearest support services based on the victim's location. Services might include the police, a nearby hospital, or available lawyers.
%Other researchers take a hardware-based approach for the victims to seek help such as voice recognition [][], safety chips on the body [][][], 
%\textit{Mention the use of personal phones or computers (VPN to hide their access to help).}








==> Tech-abuse_SmartHomes_Draft 2-3/TexFiles/Conclusion.tex <==
%Smart home devices undoubtedly have great advantages for people in terms of security, entertainment, and power efficiency.
%But, some features in smart home devices might affect someone's safety.
%Vendors need to include a diverse team to consider unintentional consequences of certain uses. 
%IPV is an example of lack of diversity in designing teams. 
%Smart home devices are designed with an assumption of absolute safety in people's houses.
Designing smart home devices with an assumption of absolute safety in homes is problematic as victims of IPV suffer in their homes, and escape plans are the only safety boat for them.
In this paper, we articulated the problem of IPV in smart homes and how it is unique.
We then proposed a framework that covers all phases of abuse in smart homes and their corresponding needs and challenges.
We explored the technical reasons that empowered abusers more than victims in current smart home devices. We discussed the recommendations offered by the research community with emphasis on their potentials and limitations.
Finally, we provided a list of desirable properties of ``abuse-resistant" smart home devices.


\iffalse

%Smart home devices undoubtedly have great advantages for people in terms of security, entertainment, and power efficiency.
%But, some features in smart home devices might affect someone's safety.
%Vendors need to include a diverse team to consider unintentional consequences of certain uses. 
%IPV is an example of lack of diversity in designing teams. 
%Smart home devices are designed with an assumption of absolute safety in people's houses.
Designing smart home devices with an assumption of absolute safety in homes is problematic as victims of IPV suffer in their homes, and escape plans are the only safety boat for them.
In this paper, we articulated IPV in smart homes and how it was different from previous approaches.
We then provided our framework that covered all phases of abuse in smart homes and their corresponding needs and challenges.
Also, we explored technical reasons in current smart home devices that empowered abusers more than victims.
Moreover, recommendations by the research community were discussed with emphasis on their potentials and limitations.
In the end, we provided desirable properties for abuse-resistant smart home devices.


\iffalse
Smart home devices have brought to us many ben-efits  such  as  advanced  security,  convenience  and  entertainment.However, these devices also have made unintended consequenceslike giving ultimate power for devices’ owners over their intimatepartners   in   the   same   household   which   might   lead   to   tech-facilitated  domestic  abuse  (tech-abuse)  as  recent  research  hasshown.  In  this  paper,wesystematizefindingsontech-abuseinsmarthomes. We show that domestic abuse or Intimate PartnerViolence (IPV) in smart homes is more effective and less risky forabusers  and  is  more  harmful  and  challenging  to  defend  againstfor victims of IPV.Wearticulateacomprehensiveanalysisofallthephasesofabuseoftech-abuseinsmarthomes,andcategorizerisksandrecommendationsineachphase.KeyinsightsresultingfromworksbothintheIPVandsmarthomecommunitiesareidentifiedandtheeffectivenessofapproachesarerelatedtotech-abuseinsmarthomes.Recommendationstodesignabuse-resistantsmarthomedevicesareproposedforallthephasesofabuse.  The  research  community  benefits  from  our  analysis  andrecommendations  to  move  forward  with  a  focus  on  filling  theblind spots of existing smart home devices’ safety measures andbuilding  new  appropriate  safety  measures  that  consider  tech-abuse  threats  in  smart  homes.
\fi

\fi

==> Tech-abuse_SmartHomes_Draft 2-3/TexFiles/Discussion.tex <==
\begin{itemize}
    \item Shortcomings and challenges
    \begin{itemize}
        \item Challenges: privacy might be violated if we add adds-on features by hackers.
        \item Technology-enabled abuse leads to fear of technology.This might hurt the industry if consumers lose trust in the products...
        \item IFTTT and trigger-action platforms challenge and opportunities.
        \item What we’ve seen time and time again is that perpetrators tend to be one step ahead in leveraging technology to use it as a tool for abuse~\cite{Wired-smartHomes_abuse}.
        \item abusers might take advantage of safety labels by not buying devices with safety features. In order to make safety labels work, legislature needs to enforce all smart home vendors include safety features and labels.
    \end{itemize}
     
    How to balance between privacy and safety.
    \item Our recommendations
    \begin{itemize}
        \item For vendors
        \begin{itemize}
            \item Adversarial training in form of abuse. So that devices can be resilient to being abused.
            \item If vendors are unable for any reason to provide abuse-resistant devices, they should at least provide guidelines for support services in case of domestic abuse cases. So, when a victim of IPV reaches out to the support services, the victim will be provided with actionable advice. 
        \end{itemize}
        \item For support services. Corona Virus Disease (\textit{aka} COVID-19) crisis has been devastating in many ways. People have lost their loved ones, their jobs and other suffered an increase in the frequency and severity of domestic abuse. The number of reported domestic abuse has been skyrocketing as shown in recent articles~\cite{DomesticAbuse_Rise_COVID}. 
        \item For law enforcement and legislators: require owners to disclose other users in the house.
        \item For users
    \end{itemize}
\end{itemize}


There have not been projects that directly focus on domestic abuse in smart homes with respect to the phases of abuse, and break down the security and privacy issues to make them easier to tackle for smart home device developers.
However, there has been noticeable efforts on similar issues.
For instance, some privacy issues arise in nursing homes when residents' families suspect mistreatment from caregivers so that they set up indoor cameras~\cite{nursing_homes_privacy}. 
This act complicates the process of data collections and violation of some stakeholders' privacy. 
States like Arizona have produced bills to regulate the use of smart devices in nursing homes.
However, there is a lack of regulations in tech-abuse, let alone SHTA. 
%This is similar to our project from the perspective of 



\subsection{Limitations}
\input{TexFiles/Limitation}

\begin{table}[!t]
	\centering
	\caption{Summary of literature for tech-abuse using smart home devices- \textit{to be edited}} 
	%\vspace{-10pt}
	\label{tab:techs}
	\begin{tabular}{|l|l|}
		\hline
		\rowcolor{Gray}
		\textbf{Focus}    &  \textbf{Tech-abuse in smart homes}        \\ \hline
	    Abuser in IPV     & \cite{SmartHome_Abuse_Category_1_paper1,SmartHome_Abuse_Category_1_paper2,SmartHome_Abuse_Category_3_paper1}   \\ \hline
		Victims in IPV & \cite{SmartHome_Abuse_Category_2_paper1,SmartHome_Abuse_Category_2_paper2,SmartHome_Abuse_Category_2_paper3,SmartHome_Abuse_Category_2_paper4,SmartHome_Abuse_Category_2_paper5,homeGuard_abuse_recognize_seekHelp,SmartHome_Abuse_Category_2_paper6}    \\ \hline
		Support services for IPV victims   & \cite{SmartHome_Abuse_Category_1_paper1,SmartHome_Abuse_Category_3_paper1,homeGuard_abuse_recognize_seekHelp}    \\ \hline
	\end{tabular}
	\label{TA_features}
	%\vspace{-10pt}
\end{table}


==> Tech-abuse_SmartHomes_Draft 2-3/TexFiles/Introduction.tex <==

Smart home devices have been adopted at a high rate in recent years. 
There is at least one smart home device in 69\% of the houses in the U.S.~\cite{SmartHome_Stat_majority_69}. 
Three in five Americans own smart home devices for security purposes in their houses~\cite{SmartHome_Security_stats}.
Many smart home devices can be programmed to do a variety of tasks. 
For example, Amazon \textit{Alexa} allows users to create their own skills such as ``start relaxing music when I get home''~\cite{Alexa_Skills}. 
This sounds entertaining for most people. 
Nevertheless, this same feature can be turned to be a great tool for eavesdropping~\cite{Alexa_Skills_Survillance}.
Recent articles in the news have reported cases of domestic abuse using smart home devices~\cite{Wired-smartHomes_abuse, News_SmartHome_Abuse}.
Smart home devices are normally designed for homes where trust is established without any dispute.
This trust assumption is not realistic as IPV cases are common globally.
According to the United Nations' 2019 global study on homicide, one in three women has been killed by their partners~\cite{UN_Report_homicide}.
The same report shows that two in three women are more likely to be killed at their home by a relative.
%Corona Virus Disease (\textit{aka} COVID-19) crisis in 2020 has been devastating in many ways. Related to this topic, the number of reported domestic abuse has been skyrocketing as shown in recent articles~\cite{}.
 



Technology-facilitated domestic abuse (tech-abuse for short) is not new.
Abusers have been using technologies like smartphones, personal computers, and GPS trackers to improve their methods of abuse. The emergence of smart home devices has just further advanced the methods that abusers would use~\cite{SmartHome_Abuse_Category_1_paper1}. 
Smart home technologies give abusers a great tool to carry out destructive activities with less effort and lower risks compared to traditional methods of abuse~\cite{SmartHome_Abuse_Category_1_paper2}. 
Still, a thorough analysis of tech-abuse in smart homes has not been conducted.

Consequently, many research projects have reacted to tech-abuse in smart homes with ways to protect the victims of Intimate Partner Violence (IPV) such as the work in~\cite{SmartHome_Abuse_Category_2_paper1, SmartHome_Abuse_Category_2_paper2, SmartHome_Abuse_Category_2_paper3}. 
Some of these projects have analyzed victims' perspectives in IPV cases through user studies and workshops. The proposed solutions to help the victims are either generic like advising IPV support services to involve cybersecurity experts for more appropriate planning or specific to one aspect of the system such as the focus of~\cite{SmartHome_Abuse_Category_2_paper3} on the usability of smart home devices. Both approaches are good to a certain extent.
Still, comprehensive analysis and solutions are missing since the issue of tech-abuse in smart homes is still emerging. 

\iffalse
In this project, we attempt to answer the following research questions:
\begin{itemize}
    \item Is tech-abuse in smart homes more rewarding, more efficient, and less risky for abusers of IPV compared to traditional abuse and other tech-abuse techniques? And is tech-abuse in smart homes more challenging and more damaging for victims of IPV compared to traditional abuse and other tech-abuse techniques?
    %\item Do smart home devices make more harm than good? 
    %\item Why are authentication mechanisms and access control systems in smart homes not abuse-resistant?
    \item Why are smart home devices not abuse-resistant?
    \item Can we break down the technical problems of smart home devices for not being abuse-resistant into smaller concrete problems for each phase of abuse?
    \item What is the state of art recommendations and suggestions that recent research in tech-abuse in smart homes has proposed?
\end{itemize}
\fi

In this paper, we develop a unified analytical framework based on characteristics of smart homes, abusers' common attributes, and possible capabilities particular to smart homes built with emerging technologies.
Our framework consists of four phases of abuse from the victim's perspective in IPV.
For each phase, we explore the goals for each stakeholder including abusers, victims, device vendors, and support services. 
Then, we review the literature with some key insights and break down security and safety challenges and needs for each phase.
%Dividing security needs to each phase helps finding concrete smaller solutions for each phase, and ideally combine all of them to have a comprehensive solutions for all the phases.
The research on ensuring human safety in smart homes is somewhat less well developed.
\begin{table*}[!t]
	\centering
	\caption{Scenario-based comparison of abuse methods. We take \textit{stalking} as an abusive action.} 
	\vspace{-8pt}
	\label{tab:techs}
	\scalebox{0.9}{
	\begin{tabular}{|l|l|}
	    \hline
	    \rowcolor{Gray}
		\textbf{Abuse type}    &  \textbf{What abusers can do}        \\ \hline
		
	   \multirow{2}{*}{Traditional abuse}&High effort:\textit{ Abusers need to spend time following the victim, be physically close, and abusive action is not immediate.} \\
         &High risk: \textit{Abusers might face resistance by victims to fight back physically, and other people might see or hear the abusive action.}\\&High benefit: \textit{Abusers can assert their power over victims.}\\ \hline
          \multirow{2}{*}{Tech-abuse}&Mid effort: \textit{Abusers  need to either be physically close to victims' devices or know the credentials, and actions are not immediate.}  \\
         &High risk: \textit{The same risk in traditional abuse applies here, and some recent defenses for victims can hold abusers accountable~\cite{Tech-abuse-smartphones-computers}.} \\&Low benefit: \textit{Restricted power for abusers as victims need to initiate activities on their phones or PCs first.} \\ \hline
          \multirow{2}{*}{SHOT}&Low effort: \textit{Abusers own the devices of the smart homes which give them full access remotely and immediately.}  \\
         &Low risk: \textit{Abusers can control their smart homes remotely and are able to delete usage history.} \\&High benefit: \textit{Abusers can control ambient surroundings of victims, and are able to discretely monitor the house.} \\ \hline
	\end{tabular}
	}
	\label{abuse_comparison}
	\vspace{-15pt}
\end{table*}

Then, we analyze the technical causes of why smart home devices empower abusers in IPV, limit victims' abilities to protect themselves, and challenge support services to provide help.
Lack of  diversity  in the designing teams, poor usability of the devices, inadequate modeling of the IPV threat in smart homes, and unreliable system functions are the main  reasons.
We then review proposed solutions by recent work to show their strengths and weaknesses as well as future directions along with desirable properties for abuse-resistant smart home devices.
To the best of our knowledge, we are the first to design a specific framework for phases of abuse in smart homes, and break down security challenges to each phase so that the research community can target the limitations of current research, and focus on a comprehensive solution that works for all the phases of abuse in smart homes.
%Our survey on existing work related to tech-abuse in smart homes is unprecedented.
\iffalse %%## this to comment out multiple lines
\hl{In this paper, we develop a *unified analytical framework based on xxxxx that considers characteristics of smart homes, *abuse types/goal?*, and possible capabilities particular to smart homes built with emerging technologies.} We answer these questions with respect to each phase of tech-abuse in smart homes. 
We first start by briefly explaining what the phase is about, and what the goals are for each stakeholder. 
Then, we show the literature in this phase with some historical information.
\hl{We then evaluate technologies in smart homes focusing on tech-abuse. Here, we consider the four phases of tech-base with respect to abusers, victims, vendors and support services, and identify the risks, efforts and means at each phase.
The research of ensuring human safety in smart homes is somewhat less well developed.}
%We then show recent findings and shortcomings from a technical standpoint. 
Lastly, we summarize recommendations and proposals to combat tech-abuse in smart homes.

In the end, we provide several design recommendations so that future research can direct their effort to the most important issues in smart home devices. 
We provide short-term and long term design recommendations with considerations to all entities involved in IPV cases such as smart home vendors, law enforcement, and users.
To the best of our knowledge, we are the first to design a specific framework for phases of abuse in smart homes, and break down security challenges to each phase. 
Our survey on existing work related to tech-abuse in smart homes is unprecedented.
\fi

\textbf{Our contributions:}
\begin{itemize}

    \item We introduce a unified analytical framework to allow structured analysis of tech-abuse in smart homes. This framework is developed from previous efforts by considering the entire lifecycle of tech-abuse, instead of smart home technologies in isolation. (Section \ref{phases})
    \item We break down the tech-abuse problems into smaller privacy and security (safety) problems in each phase. This simplifies the problem and aids in addressing it at each phase. (Section \ref{phases}) %We borrowed the notion of divide and conquer from literature. (Section \ref{phases})
    \item We observe that smart homes empower abusers and limit IPV victims' ability to protect themselves. (Section \ref{technical_causes})
    \item We summarize solutions to combat tech-abuse in smart homes to show their strengths and weaknesses in order to enhance existing ideas and guide the research community to cover the blind spots of current research. (Section \ref{summary_solutions})
    \item We systematize desirable properties to make smart home devices abuse-resistant. (Section \ref{ourProposals})
    %\item We provide technical recommendations for designing appropriate authentication mechanisms and access control approaches that are abuse-resistant.
\end{itemize}

\iffalse
In the rest of this paper, Section \ref{background} reviews some background information and related work; Section \ref{threat_model} defines the threat model; Section \ref{phases} defines our framework for phases of abuse in smart homes, and breaks down security and privacy issues concretely for each phase; Section \ref{technical_causes} reviews recent solutions and recommendations to tech-abuse in smart homes; Section \ref{ourProposals} provides our proposals for technical short and long terms designs for abuse-resistant smart homes;
%Section \ref{discussion} discusses shortcomings and challenges; 
Sections \ref{conclusion} makes a conclusion.
\fi

\iffalse % below is my witing
Smart home devices have been adopted at a high rate in recent years. 
There is at least one smart home device in 69\% of the houses in the U.S.~\cite{SmartHome_Stat_majority_69}. 
Three in five Americans own smart home devices for security purposes in their houses~\cite{SmartHome_Security_stats}.
Many smart home devices can be programmed to do a variety of tasks. 
For example, Amazon \textit{Alexa} allows users to create their own skills such as ``start relaxing music when I get home''~\cite{Alexa_Skills}. 
This sounds entertaining for most people. 
Nevertheless, this same feature can be turned to be a great tool for eavesdropping~\cite{Alexa_Skills_Survillance}.
Recent articles in the news have reported cases of domestic abuse using smart home devices~\cite{Wired-smartHomes_abuse, News_SmartHome_Abuse}.
Smart home devices are normally designed for homes where trust is established without any dispute.
However, this is not realistic as IPV cases are common globally.
In the 2019 report of homicide by the United Nations (UN), one in three women has been killed by their partners~\cite{UN_Report_homicide}.
The same report shows that two in three women are more likely to be killed at their home by a relative.
%Corona Virus Disease (\textit{aka} COVID-19) crisis in 2020 has been devastating in many ways. Related to this topic, the number of reported domestic abuse has been skyrocketing as shown in recent articles~\cite{}.
 



Technology-facilitated domestic abuse (tech-abuse for short) is not new.
Abusers have been using technologies like smartphones, personal computers, and GPS trackers to improve their methods of abuse. The emergence of smart home devices has just further advanced the methods that abusers would use~\cite{SmartHome_Abuse_Category_1_paper1}. 
Smart home technologies give abusers a great tool to carry out destructive activities with less effort and lower risks compared to traditional methods of abuse~\cite{SmartHome_Abuse_Category_1_paper2}. 
Still, a thorough analysis of tech-abuse in smart homes has not been conducted.

Consequently, many research projects have reacted to tech-abuse in smart homes with ways to protect the victims of Intimate Partner Violence (IPV) such as the work in~\cite{SmartHome_Abuse_Category_2_paper1, SmartHome_Abuse_Category_2_paper2, SmartHome_Abuse_Category_2_paper3}. 
Some of these projects have analyzed victims' perspectives in IPV cases through user studies and workshops. The proposed solutions to help the victims are either generic like advising IPV support services to involve cybersecurity experts for more appropriate plannings or specific to one aspect of the system such as the focus of~\cite{SmartHome_Abuse_Category_2_paper3} on the usability of smart home devices. Both approaches are good to a certain extent.
Still, comprehensive analysis and solutions are missing since the issue of tech-abuse in smart homes is still emerging. 

\iffalse
In this project, we attempt to answer the following research questions:
\begin{itemize}
    \item Is tech-abuse in smart homes more rewarding, more efficient, and less risky for abusers of IPV compared to traditional abuse and other tech-abuse techniques? And is tech-abuse in smart homes more challenging and more damaging for victims of IPV compared to traditional abuse and other tech-abuse techniques?
    %\item Do smart home devices make more harm than good? 
    %\item Why are authentication mechanisms and access control systems in smart homes not abuse-resistant?
    \item Why are smart home devices not abuse-resistant?
    \item Can we break down the technical problems of smart home devices for not being abuse-resistant into smaller concrete problems for each phase of abuse?
    \item What is the state of art recommendations and suggestions that recent research in tech-abuse in smart homes has proposed?
\end{itemize}
\fi

In this paper, we develop a unified analytical framework based on characteristics of smart homes, abusers' common attributes, and possible capabilities particular to smart homes built with emerging technologies.
Our framework consists of four phases of abuse from the victim's perspective in IPV.
For each phase, we explore the goals for each stakeholder including abusers, victims, device vendors, and support services. 
Then, we show the literature with some key insights and break down security and safety challenges and needs for each phase.
%Dividing security needs to each phase helps finding concrete smaller solutions for each phase, and ideally combine all of them to have a comprehensive solutions for all the phases.
The research on ensuring human safety in smart homes is somewhat less well developed.
\begin{table*}[!t]
	\centering
	\caption{Scenario-based comparison of abuse methods. We take \textit{stalking} as an abusive action.} 
	\vspace{-8pt}
	\label{tab:techs}
	\scalebox{0.9}{
	\begin{tabular}{|l|l|}
	    \hline
	    \rowcolor{Gray}
		\textbf{Abuse type}    &  \textbf{What abusers can do}        \\ \hline
		
	   \multirow{2}{*}{Traditional abuse}&High effort:\textit{ Abusers need to spend time following the victim, be physically close, and abusive action is not immediate.} \\
         &High risk: \textit{Abusers might face resistance by victims to fight back physically, and other people might see or hear the abusive action.}\\&High benefit: \textit{Abusers can assert their power over victims.}\\ \hline
          \multirow{2}{*}{Tech-abuse}&Mid effort: \textit{Abusers  need to either be physically close to victims' devices or know the credentials, and actions are not immediate.}  \\
         &High risk: \textit{The same risk in traditional abuse applies here, and some recent defenses for victims can hold abusers accountable~\cite{Tech-abuse-smartphones-computers}.} \\&Low benefit: \textit{Restricted power for abusers as victims need to initiate activities on their phones or PCs first.} \\ \hline
          \multirow{2}{*}{SHOT}&Low effort: \textit{Abusers own the devices of the smart homes which give them full access remotely and immediately.}  \\
         &Low risk: \textit{Abusers can control their smart homes remotely and are able to delete usage history.} \\&High benefit: \textit{Abusers can control ambient surroundings of victims, and are able to discretely monitor the house.} \\ \hline
	\end{tabular}
	}
	\label{abuse_comparison}
	\vspace{-15pt}
\end{table*}

Then, we analyze the technical causes of why smart home devices empower abusers in IPV, limit victims' abilities to protect themselves, and challenge support services to provide help.
Lack of  diversity  in the designing teams, poor usability of the devices, inadequate research  of the threat of IPV in smart homes, and unreliable system functions are the main  reasons.
We then review proposed solutions by recent work to show their strengths and weaknesses as well as future directions along with desirable properties for abuse-resistant smart home devices.
To the best of our knowledge, we are the first to design a specific framework for phases of abuse in smart homes, and break down security challenges to each phase so that the research community can target the blind spots of current research, and focus on a comprehensive solution that works for all the phases of abuse in smart homes.
%Our survey on existing work related to tech-abuse in smart homes is unprecedented.
\iffalse %%## this to comment out multiple lines
\hl{In this paper, we develop a *unified analytical framework based on xxxxx that considers characteristics of smart homes, *abuse types/goal?*, and possible capabilities particular to smart homes built with emerging technologies.} We answer these questions with respect to each phase of tech-abuse in smart homes. 
We first start by briefly explaining what the phase is about, and what the goals are for each stakeholder. 
Then, we show the literature in this phase with some historical information.
\hl{We then evaluate technologies in smart homes focusing on tech-abuse. Here, we consider the four phases of tech-base with respect to abusers, victims, vendors and support services, and identify the risks, efforts and means at each phase.
The research of ensuring human safety in smart homes is somewhat less well developed.}
%We then show recent findings and shortcomings from a technical standpoint. 
Lastly, we summarize recommendations and proposals to combat tech-abuse in smart homes.

In the end, we provide several design recommendations so that future research can direct their effort to the most important issues in smart home devices. 
We provide short-term and long term design recommendations with considerations to all entities involved in IPV cases such as smart home vendors, law enforcement, and users.
To the best of our knowledge, we are the first to design a specific framework for phases of abuse in smart homes, and break down security challenges to each phase. 
Our survey on existing work related to tech-abuse in smart homes is unprecedented.
\fi

\textbf{Our contributions:}
\begin{itemize}

    \item We introduce a unified analytical framework to allow structured analysis of tech-abuse in smart homes. This framework is developed from previous efforts by considering the entire lifecycle of tech-abuse, instead of smart home technologies in isolation. (Section \ref{phases})
    \item We break down the tech-abuse problems into smaller security (safety) problems in each phase to be easier to fix and identify potential means at each phase. (Section~\ref{phases}) %We borrowed the notion of divide and conquer from literature. (Section \ref{phases})
    \item We observe that smart homes empower abusers and limit victims' ability to protect themselves in IPV situations. (Section ~\ref{technical_causes})
    \item We summarize solutions to combat tech-abuse in smart homes to show their strengths and weaknesses in order to enhance existing ideas and guide the research community to cover the blind spots of current research. (Section~\ref{summary_solutions})
    \item We systematize desirable properties to make smart home devices abuse-resistant. (Section~\ref{ourProposals})
    %\item We provide technical recommendations for designing appropriate authentication mechanisms and access control approaches that are abuse-resistant.
\end{itemize}

\iffalse
In the rest of this paper, Section \ref{background} reviews some background information and related work; Section \ref{threat_model} defines the threat model; Section \ref{phases} defines our framework for phases of abuse in smart homes, and breaks down security and privacy issues concretely for each phase; Section \ref{technical_causes} reviews recent solutions and recommendations to tech-abuse in smart homes; Section \ref{ourProposals} provides our proposals for technical short and long terms designs for abuse-resistant smart homes;
%Section \ref{discussion} discusses shortcomings and challenges; 
Sections \ref{conclusion} makes a conclusion.
\fi
%my writing below
\iffalse


Smart home devices have been adopted at a high rate in recent years. 
There is at least one smart home device in 69\% of the houses in the U.S.~\cite{SmartHome_Stat_majority_69}. 
Three in five Americans own smart home devices for security purposes in their houses~\cite{SmartHome_Security_stats}.
Many smart home devices can be programmed to do a variety of tasks. 
For example, Amazon \textit{Alexa} allows users to create their own skills such as ``start relaxing music when I get home''~\cite{Alexa_Skills}. 
This sounds entertaining for most people. 
Nevertheless, this same feature can be turned to be a great tool for eavesdropping~\cite{Alexa_Skills_Survillance}.
Recent articles in the news have reported cases of domestic abuse using smart home devices~\cite{Wired-smartHomes_abuse, News_SmartHome_Abuse}.
Smart home devices are normally designed for homes where trust is established without any dispute.
This trust assumption is not realistic as IPV cases are common globally.
According to the United Nations' 2019 global study on homicide, one in three women has been killed by their partners~\cite{UN_Report_homicide}.
The same report shows that two in three women are more likely to be killed at their home by a relative.
%Corona Virus Disease (\textit{aka} COVID-19) crisis in 2020 has been devastating in many ways. Related to this topic, the number of reported domestic abuse has been skyrocketing as shown in recent articles~\cite{}.
 



Technology-facilitated domestic abuse (tech-abuse for short) is not new.
Abusers have been using technologies like smartphones, personal computers, and GPS trackers to improve their methods of abuse. The emergence of smart home devices has just further advanced the methods that abusers would use~\cite{SmartHome_Abuse_Category_1_paper1}. 
Smart home technologies give abusers a great tool to carry out destructive activities with less effort and lower risks compared to traditional methods of abuse~\cite{SmartHome_Abuse_Category_1_paper2}. 
Still, a thorough analysis of tech-abuse in smart homes has not been conducted.

Consequently, many research projects have reacted to tech-abuse in smart homes with ways to protect the victims of Intimate Partner Violence (IPV) such as the work in~\cite{SmartHome_Abuse_Category_2_paper1, SmartHome_Abuse_Category_2_paper2, SmartHome_Abuse_Category_2_paper3}. 
Some of these projects have analyzed victims' perspectives in IPV cases through user studies and workshops. The proposed solutions to help the victims are either generic like advising IPV support services to involve cybersecurity experts for more appropriate planning or specific to one aspect of the system such as the focus of~\cite{SmartHome_Abuse_Category_2_paper3} on the usability of smart home devices. Both approaches are good to a certain extent.
Still, comprehensive analysis and solutions are missing since the issue of tech-abuse in smart homes is still emerging. 

\iffalse
In this project, we attempt to answer the following research questions:
\begin{itemize}
    \item Is tech-abuse in smart homes more rewarding, more efficient, and less risky for abusers of IPV compared to traditional abuse and other tech-abuse techniques? And is tech-abuse in smart homes more challenging and more damaging for victims of IPV compared to traditional abuse and other tech-abuse techniques?
    %\item Do smart home devices make more harm than good? 
    %\item Why are authentication mechanisms and access control systems in smart homes not abuse-resistant?
    \item Why are smart home devices not abuse-resistant?
    \item Can we break down the technical problems of smart home devices for not being abuse-resistant into smaller concrete problems for each phase of abuse?
    \item What is the state of art recommendations and suggestions that recent research in tech-abuse in smart homes has proposed?
\end{itemize}
\fi

In this paper, we develop a unified analytical framework based on characteristics of smart homes, abusers' common attributes, and possible capabilities particular to smart homes built with emerging technologies.
Our framework consists of four phases of abuse from the victim's perspective in IPV.
For each phase, we explore the goals for each stakeholder including abusers, victims, device vendors, and support services. 
Then, we review the literature with some key insights and break down security and safety challenges and needs for each phase.
%Dividing security needs to each phase helps finding concrete smaller solutions for each phase, and ideally combine all of them to have a comprehensive solutions for all the phases.
The research on ensuring human safety in smart homes is somewhat less well developed.
\begin{table*}[!t]
	\centering
	\caption{Scenario-based comparison of abuse methods. We take \textit{stalking} as an abusive action.} 
	\vspace{-8pt}
	\label{tab:techs}
	\scalebox{0.9}{
	\begin{tabular}{|l|l|}
	    \hline
	    \rowcolor{Gray}
		\textbf{Abuse type}    &  \textbf{What abusers can do}        \\ \hline
		
	   \multirow{2}{*}{Traditional abuse}&High effort:\textit{ Abusers need to spend time following the victim, be physically close, and abusive action is not immediate.} \\
         &High risk: \textit{Abusers might face resistance by victims to fight back physically, and other people might see or hear the abusive action.}\\&High benefit: \textit{Abusers can assert their power over victims.}\\ \hline
          \multirow{2}{*}{Tech-abuse}&Mid effort: \textit{Abusers  need to either be physically close to victims' devices or know the credentials, and actions are not immediate.}  \\
         &High risk: \textit{The same risk in traditional abuse applies here, and some recent defenses for victims can hold abusers accountable~\cite{Tech-abuse-smartphones-computers}.} \\&Low benefit: \textit{Restricted power for abusers as victims need to initiate activities on their phones or PCs first.} \\ \hline
          \multirow{2}{*}{SHOT}&Low effort: \textit{Abusers own the devices of the smart homes which give them full access remotely and immediately.}  \\
         &Low risk: \textit{Abusers can control their smart homes remotely and are able to delete usage history.} \\&High benefit: \textit{Abusers can control ambient surroundings of victims, and are able to discretely monitor the house.} \\ \hline
	\end{tabular}
	}
	\label{abuse_comparison}
	\vspace{-15pt}
\end{table*}

Then, we analyze the technical causes of why smart home devices empower abusers in IPV, limit victims' abilities to protect themselves, and challenge support services to provide help.
Lack of  diversity  in the designing teams, poor usability of the devices, inadequate modeling of the IPV threat in smart homes, and unreliable system functions are the main  reasons.
We then review proposed solutions by recent work to show their strengths and weaknesses as well as future directions along with desirable properties for abuse-resistant smart home devices.
To the best of our knowledge, we are the first to design a specific framework for phases of abuse in smart homes, and break down security challenges to each phase so that the research community can target the limitations of current research, and focus on a comprehensive solution that works for all the phases of abuse in smart homes.
%Our survey on existing work related to tech-abuse in smart homes is unprecedented.
\iffalse %%## this to comment out multiple lines
\hl{In this paper, we develop a *unified analytical framework based on xxxxx that considers characteristics of smart homes, *abuse types/goal?*, and possible capabilities particular to smart homes built with emerging technologies.} We answer these questions with respect to each phase of tech-abuse in smart homes. 
We first start by briefly explaining what the phase is about, and what the goals are for each stakeholder. 
Then, we show the literature in this phase with some historical information.
\hl{We then evaluate technologies in smart homes focusing on tech-abuse. Here, we consider the four phases of tech-base with respect to abusers, victims, vendors and support services, and identify the risks, efforts and means at each phase.
The research of ensuring human safety in smart homes is somewhat less well developed.}
%We then show recent findings and shortcomings from a technical standpoint. 
Lastly, we summarize recommendations and proposals to combat tech-abuse in smart homes.

In the end, we provide several design recommendations so that future research can direct their effort to the most important issues in smart home devices. 
We provide short-term and long term design recommendations with considerations to all entities involved in IPV cases such as smart home vendors, law enforcement, and users.
To the best of our knowledge, we are the first to design a specific framework for phases of abuse in smart homes, and break down security challenges to each phase. 
Our survey on existing work related to tech-abuse in smart homes is unprecedented.
\fi

\textbf{Our contributions:}
\begin{itemize}

    \item We introduce a unified analytical framework to allow structured analysis of tech-abuse in smart homes. This framework is developed from previous efforts by considering the entire lifecycle of tech-abuse, instead of smart home technologies in isolation. (Section \ref{phases})
    \item We break down the tech-abuse problems into smaller privacy and security (safety) problems in each phase. This simplifies the problem and aids in addressing it at each phase. (Section \ref{phases}) %We borrowed the notion of divide and conquer from literature. (Section \ref{phases})
    \item We observe that smart homes empower abusers and limit IPV victims' ability to protect themselves. (Section \ref{technical_causes})
    \item We summarize solutions to combat tech-abuse in smart homes to show their strengths and weaknesses in order to enhance existing ideas and guide the research community to cover the blind spots of current research. (Section \ref{summary_solutions})
    \item We systematize desirable properties to make smart home devices abuse-resistant. (Section \ref{ourProposals})
    %\item We provide technical recommendations for designing appropriate authentication mechanisms and access control approaches that are abuse-resistant.
\end{itemize}

\iffalse
In the rest of this paper, Section \ref{background} reviews some background information and related work; Section \ref{threat_model} defines the threat model; Section \ref{phases} defines our framework for phases of abuse in smart homes, and breaks down security and privacy issues concretely for each phase; Section \ref{technical_causes} reviews recent solutions and recommendations to tech-abuse in smart homes; Section \ref{ourProposals} provides our proposals for technical short and long terms designs for abuse-resistant smart homes;
%Section \ref{discussion} discusses shortcomings and challenges; 
Sections \ref{conclusion} makes a conclusion.
\fi
\fi
\fi %end of my writing

==> Tech-abuse_SmartHomes_Draft 2-3/TexFiles/Limitation.tex <==
Limitations and future work.

==> Tech-abuse_SmartHomes_Draft 2-3/TexFiles/Living.tex <==

\begin{table}[!t]
	\centering
	\caption{Summary of security and safety needs for each phase} 
	\vspace{-8pt}
	\label{tab:techs}
	\scalebox{0.9}{%% This reduces the whole table, fonts and dimensions
	\begin{tabular}{|p{8.5cm}|}
		\hline
		
	%	\\ \hline
	%	\hline
	\rowcolor{Gray}
		\textbf{Acquiring}            \\ \hline
		
		\begin{itemize}
        \item Capabilities of smart home devices should be shown (similar to nutrition labels), including safety measures.
        %\item Vendors should provide guidelines to support services
        \item Authentication  mechanisms should consider   multi-users' environments.
        \item Setup processes should consider involving other occupants. 
    \end{itemize}       \\ \hline
    	
    	\rowcolor{Gray}
    	\textbf{Recognizing}            \\ \hline
		
		\begin{itemize}
        \item Implementing continuous authentication to differentiate between users and to include context.
        \item Implementing context-aware access control can help mitigate IPV.
        \item Using nudges to show users data flow and corresponding purposes can raise victms' awareness of abuse risk.
        \item Devices should give equal access power to users in the same home if they are partners.
         \end{itemize}       \\ \hline
    	
    	\rowcolor{Gray}
    	\textbf{Acting}            \\ \hline
		
		\begin{itemize}
        \item Solid security logging can help create evidence and protect victims of IPV.
        \item Vendors should consider adding ways to facilitate reporting domestic abuse if identified.
       % Ways  to  share  this  with  law enforcement when abuse is identified (modes of operations)
        \item The research community should aim to develop adversarial models of tech-abuse for different devices. Voice and image recognition or traffic analysis may be sources of data, but user privacy needs to be taken into account.
        %Adversarial training so that   could   recognize   abuse through   image   recognition   or   voice   recognition
        \item Access control needs to be reliable and immediate.
    \end{itemize}       \\ \hline
    		
    	\rowcolor{Gray}
    	\textbf{Living}            \\ \hline
		
		\begin{itemize}
        \item Current cybersecurity measures may be good enough. 
        \item There is a need to raise user awareness of cybersecurity hygiene.
        \item Restraining orders need to account for smart home devices.
    \end{itemize}       \\ \hline
	\end{tabular}
	}
	\label{Table_phases_summary_needs}
	\vspace{-10pt}
\end{table}

%When abuse has been recognized and victims have acted upon it to seek help or escape, victims 
In this phase, victims seek to establish a new life without their abusers. They may move to a new place, revoke abusers' access to smart homes, or have a restraining order on their abusers. 
Sharing access to smart home devices might get tricky as it is not clear who should ``own" the shared device after separation. 
In addition, living completely independently might be impossible if the victim and the abuser have kids together~\cite{Stories_survivors_IPV}.

It is important to notice that separating procedures take a long time. Victims of IPV need to ensure they are safe during that period~\cite{Seperating_takes_time}.
Transfer of ownership of smart home devices needs to be accounted for in the design stages, so that when victims of IPV want to revoke abusers' access, the process is easy and takes effect immediately~\cite{challenges_safety_smart_Environments}.
In this phase, the abuser should have lost access to the smart home devices, which they used to carry out harmful actions on  towards the victim. The abuser might try to regain access. 
The goal is to teach the victim how to revoke access from the abuser and keep access to the smart home devices private and secure. 
Particularly, victims of IPV need to be knowledgeable about privacy and security best practices to protect themselves~\cite{Stories_survivors_IPV}.

Legally, lawyers of the victims of IPV have difficulties including the access to smart home devices in restraining orders to stop abusers from attempting to regain access~\cite{NY_Times_Tech_Abuse}.
Traditionally, restraining orders account for the victim's home and work buildings.
But, abusers exploiting SHOT do not to be in proximity to carry out harm. 
This adds complexities in writing restraining orders for lawyers and judges as well.
Moreover, security tools need to be effective in terms of timeliness and reliability so that victims can trust the devices to perform as expected~\cite{Access_control_not_working}.
We foresee the need for reliable access control in smart home devices so that revoking requests can be immediate even if usability is slightly compromised. 

Table \ref{Table_phases_summary_needs} summarizes the needs and potential solutions for each phase in our framework.
None of the previous work has considered all the phases in their designs which results in missing abuse-resistant smart home devices.

\iffalse
\textbf{Summary  of security  and  privacy  needs for each phase}:
\begin{itemize}
    \item Acquiring
    \begin{itemize}
        \item Capabilities of smart home devices should be shown as nutrition labels, including safety measures.
        %\item Vendors should provide guidelines to support services
        \item Authentication  mechanisms should consider   multi-users environments.
        \item Setup processes should consider involving other occupants. 
    \end{itemize}
    %,   (most impactful: vendors, regulations)
    \item Recognizing
    \begin{itemize}
        \item \textit{Implementing continuous authentication to differentiate between users \textbf{We'll add evidence}}
        \item Implementing context-aware access control can help mitigate IPV.
        \item Using nudges to show users data flow and corresponding purposes can raise awareness to victims of IPV.
        \item Devices should give equal access power to users of the same home if they are partners.
    \end{itemize}
     % ,  ,    (most impactful: vendors, regulations, users)
    \item Acting
    \begin{itemize}
        \item Solid security logging can help create evidence and protect victims of IPV.
        \item Vendors should consider adding ways to facilitate reporting domestic abuse if identified.
       % Ways  to  share  this  with  law enforcement when abuse is identified (modes of operations)
        \item The research community should aim to develop adversarial models of tech-abuse for different devices. Voice and image recognition or traffic analysis can be the source of data.
        %Adversarial training so that   could   recognize   abuse through   image   recognition   or   voice   recognition
        \item Access control needs to be reliable and immediate.
    \end{itemize}
    %(most impactful influence: regulations, )
    \item Living
    \begin{itemize}
        \item Current cybersecurity measures can be good enough 
        \item There is a need to raise user awareness of cybersecurity hygiene.
        \item Restraining orders need to account for smart home devices.
    \end{itemize}
 %(users,support services).
\end{itemize}
\fi



%The research community should focus on the first three phases as they need the most of the attention currently.

\iffalse % my writing is below, Malek's is above
\begin{table}[!t]
	\centering
	\caption{Summary of security and safety needs for each phase} 
	\vspace{-8pt}
	\label{tab:techs}
	\scalebox{0.9}{%% This reduces the whole table, fonts and dimensions
	\begin{tabular}{|p{8.5cm}|}
		\hline
		
	%	\\ \hline
	%	\hline
	\rowcolor{Gray}
		\textbf{Acquiring}            \\ \hline
		
		\begin{itemize}
        \item Capabilities of smart home devices should be shown as nutrition labels, including safety measures.
        %\item Vendors should provide guidelines to support services
        \item Authentication  mechanisms should consider   multi-users environments.
        \item Setup processes should consider involving other occupants. 
    \end{itemize}       \\ \hline
    	
    	\rowcolor{Gray}
    	\textbf{Recognizing}            \\ \hline
		
		\begin{itemize}
        \item Implementing continuous authentication to differentiate between users to build context.
        \item Implementing context-aware access control can help mitigate IPV.
        \item Using nudges to show users data flow and corresponding purposes can raise awareness to victims of IPV.
        \item Devices should give equal access power to users of the same home if they are partners.
         \end{itemize}       \\ \hline
    	
    	\rowcolor{Gray}
    	\textbf{Acting}            \\ \hline
		
		\begin{itemize}
        \item Solid security logging can help create evidence and protect victims of IPV.
        \item Vendors should consider adding ways to facilitate reporting domestic abuse if identified.
       % Ways  to  share  this  with  law enforcement when abuse is identified (modes of operations)
        \item The research community should aim to develop adversarial models of tech-abuse for different devices. Voice and image recognition or traffic analysis can be the source of data.
        %Adversarial training so that   could   recognize   abuse through   image   recognition   or   voice   recognition
        \item Access control needs to be reliable and immediate.
    \end{itemize}       \\ \hline
    		
    	\rowcolor{Gray}
    	\textbf{Living}            \\ \hline
		
		\begin{itemize}
        \item Current cybersecurity measures can be good enough. 
        \item There is a need to raise user awareness of cybersecurity hygiene.
        \item Restraining orders need to account for smart home devices.
    \end{itemize}       \\ \hline
	\end{tabular}
	}
	\label{Table_phases_summary_needs}
	\vspace{-10pt}
\end{table}

%When abuse has been recognized and victims have acted upon it to seek help or escape, victims 
In this phase, victims seek to establish a new life without their abusers such as moving to a new place, revoking abusers' access to smart homes, or having a restraining order on their abusers. 
Sharing access to smart home devices might get tricky as it is not clear who should own shared devices after separation. 
In addition, living completely independently might be impossible if the victim and the abuser share kids~\cite{Stories_survivors_IPV}.

It is important to notice that separating procedures take a long time and victims of IPV need to keep themselves safe during that period~\cite{Seperating_takes_time}.
Changing owners of smart home devices needs to be accounted for in the design stages so that when victims of IPV want to revoke abusers' access, the process should be immediate and easy~\cite{challenges_safety_smart_Environments}.
In this phase, the abuser should have lost access to the smart home devices that were used to carry out harmful actions on their intimate partner (the victim), and the abuser might try to regain access. 
The goal is to train the victim on how to revoke access from the abuser and keep access to the smart home devices private and secure. 
Particularly, victims of IPV need to be knowledgeable about privacy and security practices to protect themselves~\cite{Stories_survivors_IPV}.

Legally, lawyers of the victims of IPV have difficulties including the access to smart home devices in restraining orders to stop abusers from attempting to regain access~\cite{NY_Times_Tech_Abuse}.
Traditionally, restraining orders account for the victim's home and work buildings.
But, abusers exploiting SHOT do not to be in proximity to carry out harm. 
This adds complexities in writing restraining orders for lawyers and judges as well.
Moreover, security tools need to be effective in terms of timeliness and reliability so that victims can trust the devices to perform as expected~\cite{Access_control_not_working}.
We foresee the need for reliable access control in smart home devices so that revoking requests can be immediate even if usability is slightly compromised. 

Table \ref{Table_phases_summary_needs} summarizes the needs and potential solutions for each phase in our framework.
None of the previous work has considered all the phases in their designs which results in missing abuse-resistant smart home devices.

\iffalse
\textbf{Summary  of  security  and  privacy  needs for each phase}:
\begin{itemize}
    \item Acquiring
    \begin{itemize}
        \item Capabilities of smart home devices should be shown as nutrition labels, including safety measures.
        %\item Vendors should provide guidelines to support services
        \item Authentication  mechanisms should consider   multi-users environments.
        \item Setup processes should consider involving other occupants. 
    \end{itemize}
    %,   (most impactful: vendors, regulations)
    \item Recognizing
    \begin{itemize}
        \item \textit{Implementing continuous authentication to differentiate between users \textbf{We'll add evidence}}
        \item Implementing context-aware access control can help mitigate IPV.
        \item Using nudges to show users data flow and corresponding purposes can raise awareness to victims of IPV.
        \item Devices should give equal access power to users of the same home if they are partners.
    \end{itemize}
     % ,  ,    (most impactful: vendors, regulations, users)
    \item Acting
    \begin{itemize}
        \item Solid security logging can help create evidence and protect victims of IPV.
        \item Vendors should consider adding ways to facilitate reporting domestic abuse if identified.
       % Ways  to  share  this  with  law enforcement when abuse is identified (modes of operations)
        \item The research community should aim to develop adversarial models of tech-abuse for different devices. Voice and image recognition or traffic analysis can be the source of data.
        %Adversarial training so that   could   recognize   abuse through   image   recognition   or   voice   recognition
        \item Access control needs to be reliable and immediate.
    \end{itemize}
    %(most impactful influence: regulations, )
    \item Living
    \begin{itemize}
        \item Current cybersecurity measures can be good enough 
        \item There is a need to raise user awareness of cybersecurity hygiene.
        \item Restraining orders need to account for smart home devices.
    \end{itemize}
 %(users,support services).
\end{itemize}
\fi



%The research community should focus on the first three phases as they need the most of the attention currently.
\fi

==> Tech-abuse_SmartHomes_Draft 2-3/TexFiles/Phases_of_Abuse.tex <==




Recent studies have shown that domestic abuse takes different phases.
The phases of abuse depend on the methods that abusers take. 
Walker explains a few phases of traditional abuse where abusers do not use technologies in their actions~\cite{Walker_Traditional_abuse}.
Matthews et al. consider that three phases of abuse are the most appropriate for tech-abuse: physical control, escape, and life apart~\cite{Stories_survivors_IPV}.
In the physical control phase, both abusers and victims of IPV can access shared devices within close proximity. 
In the escape phase, abusers try to retain their access, while victims try to revoke the abusers' access. 
This is the most dangerous phase since abusers normally escalate their aggressiveness before they lose control~\cite{SmartHome_Abuse_Category_2_paper4}. 
The last phase is life apart where victims of IPV try to move on without any contact with their abusers. 
In order for any solution to be effective in combating domestic abuse, whether traditional or tech-based, it needs to address protection in all four phases of abuse, as each phase calls for specific actions. 
Two challenges are missing in recent papers: (1) Who configures smart home devices is a key component in attaining control or preventing control, and (2) Some victims can not recognize the abuse itself or the tools that the abusers use~\cite{AugustLock_Analysis_owner_Capabilities_example,RecognizingAbuse_Traditional,RecognizingAbuse_Traditional_2}.
Therefore, there is a need to redesign the abuse framework to include the missing components in SHOT.
%\vspace{-5pt}

As illustrated in Figure \ref{phases_figure}, we design our framework that consists of four phases of SHOT from the victim's perspective: acquiring smart home devices, recognizing abusive behaviors by intimate partners using these devices, acting upon these behaviors, and living after separation from abusive partners. 
In the acquiring phase, whoever configures the device will have more power to control it compared to other users in the same home.
This is important as the owner account is the decision maker because he or she can manage all users, log usage history, and revoke access~\cite{AugustLock_Analysis_owner_Capabilities_example}. 
In the recognizing phase, victims do not always recognize abusive actions by their partners as abusers normally hide their tools~\cite{RecognizingAbuse_Traditional,RecognizingAbuse_Traditional_2}. 
For instance, recently on the news, a husband confronted his wife over a private conversation that she had with her mom while she was not aware that he was listening~\cite{News_SmartHome_Abuse}.
This example of eavesdropping shows that the IPV victim did not recognize the abuse.
In the acting phase, IPV victims try to reach out for help and record evidence of abuse stealthily to protect themselves.
Lastly, victims and abusers will live separately, and this phase will explore the tools that victims can use to keep their smart home safe. 
Figure \ref{phases_figure} shows the important goals in each phase for each entity involved in IPV.
For example, IPV victims in the recognizing phase aim to look for signs of abuse such as suspicious activities by the smart home devices.
It would be greatly helpful if devices were equipped with features to help victims confirm such suspicions.
Unfortunately, this is not the feasible with current smart home devices.

\subsection{Acquiring a smart home device}
\input{TexFiles/Acquiring}
\subsection{Recognizing abuse in smart homes}
\input{TexFiles/Recognizing}
\subsection{Acting upon abuse in smart homes}
\input{TexFiles/Acting}
\subsection{Living after abuse is identified in smart homes}
\input{TexFiles/Living}



==> Tech-abuse_SmartHomes_Draft 2-3/TexFiles/Previous_Solutions_Summary.tex <==

Recent research and government efforts related to domestic abuse fall in three categories: (1) restraining abusers, (2) developing resources for victims to raise awareness about abuse and facilitate communications with support services, and (3) training personnel involved in countering IPV.
These measures generally help hold abusers accountable and empower victims to protect themselves. 
However, we see a lack of similar initiatives in combating IPV in smart homes~\cite{SmartHome_Abuse_Category_1_paper1}.
In this section, we explore the efforts of the research community to combat IPV that exploit smart home technologies.
%In this section, we explore the efforts by the research community, organizations that fight IPV, and  to help combat IPV that exploit smart home technologies. 
%news articles

Our goal is to compare the proposed solutions and identify similarities, differences, and future directions.
Table \ref{literature_solutions} manifests our summarized list of recent solutions and our assessment of their potential and limitations. 
It also illustrates similarities and differences as well as conflicts in different phases.
It is worth noting that the recommendations in the literature are mostly directed to vendors or support services generically.
Freed et al. discuss the issue of a lack of actionable instructions~\cite{SmartHome_Abuse_Category_2_paper4}.
%Vendors should provide detailed guidelines to support services where help can be provided to victims of IPV.
%Furthermore, training support services periodically can help keep personnel up-to-date with recent technologies abusers use.
We do not provide an exhaustive list of the proposed solutions due to the page limit for the paper.
We selected a sample of solutions highlighting the lack of complete, transparent, private, and reliable solutions in the market.

We see conflicting solutions in Table \ref{summary_solutions} because these solutions were designed without consideration of the phases of abuse in smart homes. 
An effective solution to one phase might not work for another phase.
Our framework will assist future designs to prevent conflicting solutions and design a solution that works in all the phases.
Another reasonable assumption is that devices will have modes of operations. So that if abuse is suspected, the device mode will switch to an abusive mode where priorities and functionalities change.
For example, the SmartThings hub has modes of operations such as home, away, and night~\cite{smartthings}.
Modes of operation can include a safety mode, which can be triggered by abusive behaviors.
Future research can address the following questions: (1) What could trigger an abusive mode?, (2) Are these triggers preventable?,
%How reliable are the triggers?  
(3) Who should be contacted for help?, and
(4) Does the abusive mode affect user experience in non-abusive environments?


% MAlek's above - my writing is below
\iffalse
Recent actions concerning domestic abuse by governments and researchers are mainly in three directions: restraining abusers, developing resources for victims to raise awareness about abuse and facilitate communications with support services, and training personnel involved in countering IPV.
These measures generally help hold abusers accountable and empower victims to protect themselves. 
However, we see a lack of similar initiatives in combating IPV in smart homes~\cite{SmartHome_Abuse_Category_1_paper1}.
In this section, we explore the efforts of the research community to combat IPV that exploit smart home technologies
%In this section, we explore the efforts by the research community, organizations that fight IPV, and  to help combat IPV that exploit smart home technologies. 
%news articles

Our goal is to review the proposed solutions and compare them to find similarities, differences, and future directions.
Table \ref{literature_solutions} manifests our summarized list of recent solutions and our analysis of their potentials and limitations. 
It also illustrates similarities and differences as well as conflicts in different phases.
It is worth noting that the recommendations in the literature are mostly directed to vendors or support services generically.
Freed et al. discuss the issue of a lack of actionable instructions~\cite{SmartHome_Abuse_Category_2_paper4}.
%Vendors should provide detailed guidelines to support services where help can be provided to victims of IPV.
%Furthermore, training support services periodically can help keep personnel up-to-date with recent technologies abusers use.
We did not include all proposed solutions in the literature due to the page limitation.
We chose a subset of them to emphasize the lack of complete, transparent, private, and reliable solutions in recent work.

%% Commented out  ####################################
\iffalse
\begin{itemize}
    \item No solution to fix all, solutions need to fix all the issues in all phases of abuse with respect to the balance between privacy and safety.
    \item List all solutions
    \item Agreed upon solutions
    \item conflicted solutions generally
    \item conflicted solutions based on different entities (abuser, victims, support)
    \item Short term vs long term
    \item doable vs hard
    \item cost
\end{itemize}
\fi 
%% Commented out  ####################################
 
%#######&&&&^^^^^^^^^^^ MENTION that the table does not have all solutions but a subset of them for showing examples of agreement and conflicting.
We see conflicting solutions in Table \ref{summary_solutions} because these solutions were designed without consideration of the phases of SHOT. 
An effective solution to one phase might not work for another phase.
Our framework will assist future designs to prevent conflicting solutions and design a solution that works in all the phases.
Another reasonable assumption is that vendors will make their devices have modes of operations. So that if abuse is suspected, the device mode will switch to an abusive mode where priorities and functionalities change.
For example, the SmartThings hub has modes of operations such as home, away, and night~\cite{smartthings}.
Modes of operations can add a safety mode which can be triggered by abusive behaviors.
The questions that need answers by future research are: What triggers the abusive mode? Are these triggers preventable? 
How reliable are the triggers?  
Who should be contacted for help?
Does the abusive mode affect user experience in non-abusive environments?
\fi

==> Tech-abuse_SmartHomes_Draft 2-3/TexFiles/Proposal.tex <==
After revising recent proposals and recommendations in Section \ref{summary_solutions}, it is clear that desirable properties are missing for developing abuse-resistant devices. 
%First, we emphasize the importance in approaching the issues in tech-abuse in smart homes with different focuses. 
Based on our framework and analysis of the literature in Section \ref{phases}, we recommend a list of \textbf{desirable properties for designing abuse-resistant smart home devices below.}
%\hl{Desirable properties for designing abuse-resistant smart home devices may be defined and enforced at each of the phases as described in Section} \ref{phases} in SHTA.
\begin{itemize}
\item \textbf{Completeness:}  A complete solution accounts for all phases of abuse. Technical, legal, and ethical perspectives need to be considered for a complete solution.
\item \textbf{Transparency:} This helps create context and ideally will help raise awareness and prevent abuse~\cite{Access_control_not_working,IBM_tech_abuse_design}.
%% Add more info about the properties either references or not and 
\item \textbf{Equal access for partners:} Devices should be designed for multiple users by default. 
For example, when equal partners share a smart home, both should have equal access power to the devices. 
This also calls for understanding the technical gaps between users, so that vendors can design appropriate devices even for less tech-savvy users.
\item \textbf{Privacy-preserving safety features:} Modes of operations should account for abusive triggers and environments. 
This helps maintain utility for non-abusive environments.
\item \textbf{Reliability:} Smart home devices should prioritize safety over convenience.
For example, revoking access should be considered as an important low-latency request. %So that if an IPV victim revokes an abuser's access, this request needs to be reliable.
This also can help victims create a legal case when abuse is identified.
%\item 
\iffalse
\item A complete solution accounts for all phases of abuse.
\item Technical, legal and ethical perspectives need to considered for a complete solution.
\item Devices should be designed for multi-user by default.
\item Transparency: this helps create context and ideally will help utilize it to raise awareness and prevent abuse.
\item Modes of operations should account for abusive triggers and environments. This helps maintain utility for non-abusive environments.
\item Acquiring and recognizing phases call for innovative solutions as they are relatively untouched by researchers compared to other phases.
\fi
\end{itemize}

\iffalse
A figure to show that what can be done now with accessible resources, in the near future for vendors and others, far future such as legislation similar to the ones already conducted with respect to the complexities of smart home devices.

\begin{itemize}
    \item Architecture: hub-based, cloud-based, or device-based
    \item per device, per capability solutions
    \item Modes of operations for devices
    \item API only approved after claims to preserve privacy, might harm  safety 
    \item Categorize requests of smart home devices
    \item Critical requests need to be approved by both occupants, similar to joint credit cardholders.
\end{itemize}
\fi


\iffalse

After revising recent proposals and recommendations in Section \ref{summary_solutions}, it is clear that desirable properties are missing for developing abuse-resistant devices. 
%First, we emphasize the importance in approaching the issues in tech-abuse in smart homes with different focuses. 
Based on our framework and analysis of literature in Section \ref{phases}, we discuss \textbf{desirable properties for designing abuse-resistant smart home devices below.}
%\hl{Desirable properties for designing abuse-resistant smart home devices may be defined and enforced at each of the phases as described in Section} \ref{phases} in SHTA.
\begin{itemize}
\item \textbf{Completeness:}  a complete solution accounts for all phases of abuse. Technical, legal, and ethical perspectives need to be considered for a complete solution.
\item \textbf{Transparency:} this helps create context and ideally will help raise awareness and prevent abuse~\cite{Access_control_not_working,IBM_tech_abuse_design}.
%% Add more info about the properties either references or not and 
\item \textbf{Equal access for partners:} devices should be designed for multi-user by default. 
For example, when equal partners share a smart home, both should have equal access power to the devices. 
This also calls for understanding the technical gaps between users so that vendors can design appropriate devices, even for not tech-savvy users.
\item \textbf{Privacy-preserving safety features:} modes of operations should account for abusive triggers and environments. 
This helps maintain utility for non-abusive environments.
\item \textbf{Reliability:} smart home devices should prioritize safety over convenience.
This also helps victims create a legal case when abuse is identified.
%\item 
\iffalse
\item A complete solution accounts for all phases of abuse.
\item Technical, legal and ethical perspectives need to considered for a complete solution.
\item Devices should be designed for multi-user by default.
\item Transparency: this helps create context and ideally will help utilize it to raise awareness and prevent abuse.
\item Modes of operations should account for abusive triggers and environments. This helps maintain utility for non-abusive environments.
\item Acquiring and recognizing phases call for innovative solutions as they are relatively untouched by researchers compared to other phases.
\fi
\end{itemize}

\iffalse
A figure to show that what can be done now with accessible resources, in the near future for vendors and others, far future such as legislation similar to the ones already conducted with respect to the complexities of smart home devices.

\begin{itemize}
    \item Architecture: hub-based, cloud-based, or device-based
    \item per device, per capability solutions
    \item Modes of operations for devices
    \item API only approved after claims to preserve privacy, might harm  safety 
    \item Categorize requests of smart home devices
    \item Critical requests need to be approved by both occupants, similar to joint credit cardholders.
\end{itemize}
\fi


\fi

==> Tech-abuse_SmartHomes_Draft 2-3/TexFiles/Recognizing.tex <==



Parkin et al. and Matthews et al. have considered three phases of tech-abuse~\cite{SmartHome_Abuse_Category_2_paper3,Stories_survivors_IPV}.
The first two phases are physical control and escape. 
In this paper, we argue that their approaches miss a very important phase from the victim's perspective. In their approach, physical control means that the abuser still has physical access to the devices in the house. 
The problem here comes from the fact that victims of IPV struggle to recognize abuse~\cite{AugustLock_Analysis_owner_Capabilities_example,RecognizingAbuse_Traditional,RecognizingAbuse_Traditional_2,social_media_IPV}. 
With traditional methods of abuse or tech-abuse in smartphones or computers, organizations have come up with guidelines to help victims recognize patterns or signs of abuse~\cite{NDVH_abuse_signs}. Goulden et al. explain some challenges of living with interpersonal data. 
The authors conduct a few studies to measure accountability and observability leading to the need for new careful designs of smart home technologies to prevent unintended consequences such as tech-abuse~\cite{SmartHome_Abuse_Category_2_paper5}.


The research community has not paid attention to techniques that can assist victims of IPV with recognizing abuse in smart homes. 
Device vendors can develop tools to alarm users of the house with respect to whom these alarms should appear. %with adversarial training 
Suppose a smart home device is equipped with safety features to recognize potential domestic abuse. The context-aware device could show warnings --such as playing some sounds to explain some data flows for users in the house-- to warn of remote access~\cite{SmartHome_Abuse_Category_2_paper1,SmartHome_Abuse_Category_1_paper2}.


A context-aware authorization scheme is a great option to help victims of IPV recognize abuse signals. 
Ghosh et al. propose \textit{softAuthZ} that is an authorization scheme in smart homes. 
It incorporates soft security attributes such as the trust level between users and other contextual variables to support authorization management~\cite{softAuthZ_ContextAware}.
IPV victims can use \textit{softAuthZ} to understand the sources of requests and the contextual information.
%For example, \textit{softAuthZ} could be used to detect signals of abuse if its soft security mechanisms considered the source of requests and users' locations into their context for evaluating requests.
Moreover, using voice recognition to differentiate between users can help prevent excessive control power that abusers take advantage of~\cite{SmartHome_Abuse_Category_2_paper1}. 
Voice recognition can be used as well to notify the appropriate party if abuse is suspected. 
This calls for a continuous authentication mechanism so that the voice assistant can tell who is sending the commands and who might be abused.
Work like~\cite{voice_assistant_continuousAuthntication} can be utilized to accommodate the needs of distinguishing users.

The goals in this phase are to mitigate abuser's harmful activities, notify victims of signs for potential abusive activities, and assist support services. 
First, implementing context-aware dynamic firewalls can limit abusers' excessive control power in IPV settings~\cite{SmartHome_Abuse_Category_2_paper1}.
Second, empowering IPV victims by making support resources reachable through smart home devices, enhancing data flow visualization  so that users can make sense of activities in their home, and implementing context-aware dynamics firewalls~\cite{SmartHome_Abuse_Category_2_paper1,SmartHome_Abuse_Category_2_paper3}. 
Last, smart home vendors can provide front-liners in support services with guidelines on how to help victims of IPV in SHOT~\cite{SmartHome_Abuse_Category_1_paper1}.




\iffalse
Parkin et al. and Matthews et al. have considered three phases of tech-abuse~\cite{SmartHome_Abuse_Category_2_paper3,Stories_survivors_IPV}.
The first two phases are physical control and escape. 
In this paper, we argue that their approaches miss a very important phase from the victim's perspective. In their approach, physical control means that the abuser still has physical access to the devices in the house.
The problem here comes from the fact that victims of IPV struggle to recognize abuse~\cite{AugustLock_Analysis_owner_Capabilities_example,RecognizingAbuse_Traditional,RecognizingAbuse_Traditional_2,social_media_IPV}. 
With traditional methods of abuse or tech-abuse in smartphones or computers, organizations have come up with guidelines to help victims recognize patterns or signs of abuse~\cite{NDVH_abuse_signs}. Goulden et al. explain some challenges of living with interpersonal data. 
The authors conduct a few studies to measure accountability and observability leading to the need for new careful designs of smart home technologies to prevent unintended consequences such as tech-abuse~\cite{SmartHome_Abuse_Category_2_paper5}.


The research community has not paid attention to techniques that can assist victims of IPV with recognizing abuse in smart homes.
Device vendors can develop tools to alarm users of the house with respect to whom these alarms should appear. %with adversarial training 
Suppose a smart home device is equipped with safety features to recognize potential domestic abuse. The context-aware device could show warnings --such as playing some sounds to explain some data flows for users in the house-- to warn of remote access~\cite{SmartHome_Abuse_Category_2_paper1,SmartHome_Abuse_Category_1_paper2}.
A context-aware authorization scheme is a great option to help victims of IPV recognize abuse signals. For example, \textit{softAuthZ} could be used to detect signals of abuse if its soft security mechanisms considered the source of requests and users' locations into their context for evaluating requests~\cite{softAuthZ_ContextAware}.
Moreover, using voice recognition to differentiate between users can help prevent excessive control power that abusers take advantage of~\cite{SmartHome_Abuse_Category_2_paper1}. 
Voice recognition can be used as well to notify the appropriate party if abuse is suspected.
This calls for a continuous authentication mechanism so that the voice assistant can tell who is sending the commands and who might be abused.
Work like~\cite{voice_assistant_continuousAuthntication} can be utilized to accommodate the needs of distinguishing users.

The goals in this phase are to mitigate abuser's harmful activities, notify victims of signs for potential abusive activities, and assist support services. 
First, implementing context-aware dynamics firewalls can limit abusers' excessive control power in IPV settings~\cite{SmartHome_Abuse_Category_2_paper1}.
Second, empowering IPV victims by making support resources reachable through smart home devices, enhancing data flow visualization so that users can make sense of activities in their home, and implementing context-aware dynamics firewalls~\cite{SmartHome_Abuse_Category_2_paper1,SmartHome_Abuse_Category_2_paper3}.
%Second, empowering victims of IPV by making support resources reachable through smart home devices, enhancing visualization of data flows so that users can make sense of activities in their house, and implementing context-aware dynamics firewalls~\cite{SmartHome_Abuse_Category_2_paper1,SmartHome_Abuse_Category_2_paper3}. 
Last, smart home vendors can provide front-liners in support services with guidelines on how to help victims of IPV in SHOT~\cite{SmartHome_Abuse_Category_1_paper1}.
\fi



==> Tech-abuse_SmartHomes_Draft 2-3/TexFiles/TechnicalCasues.tex <==
In this section, we investigate why current smart home devices empower abusers in IPV from a technical standpoint. We explore how they limit victims' abilities to protect themselves and how they may obstruct support services.
The literature shows that smart home device designers do not consider multi-user environments in the authentication and access control mechanisms, which leads to empowering abusers over victims of IPV~\cite{Access_control_not_working,European_Cybersecurity_report_imbalanceControlProblem}. 

\textbf{The blackbox nature of smart home devices is troublesome.} Litão explains how this blackbox nature inhibits users' abilities to understand the data flow and how this plays a big role in the unequal control power between intimate partners~\cite{SmartHome_Abuse_Category_2_paper1}.
The majority of smart home devices do not offer an interface on the same device. Generally, they use of smartphones for authentication, access control, and privacy settings~\cite{European_Cybersecurity_report_imbalanceControlProblem}. 

\textbf{Recent security research did not consider UI-Adversary in their threat models.}
Slupska conducted a thorough analysis of 44 research papers about security in smart homes.She found that none of them had considered IPV in their threat models~\cite{feminist_Cybersecurity}.
Recent research focused on the same security issues as in personal computers and smartphones. 
Smart homes are different from traditional technology: Social complexities and potential unequal access are extremely important to the safety of users~\cite{European_Cybersecurity_report_imbalanceControlProblem}.

\textbf{Access control in smart home devices is not reliable.}
Janes et al. evaluate 19 popular smart home devices and find that 16 of them struggle to revoke access from previously authorized users even after changing passwords or explicitly revoking their access~\cite{Access_control_not_working}. 
The findings in~\cite{Access_control_not_working} show that these changes are either not enforced at all or do not take effect immediately, making the majority of the smart home devices not reliable when it comes to protecting victims.


\textbf{Smart home devices are not designed for a multi-user environment.}
Recent work discusses why current smart home devices are not designed for multiple users. The authors of ~\cite{multi-user-problem-smart-home,Rethinking_Access_control_Authnetication} conducted user studies to qualitatively analyze users' needs in smart homes. 
The findings call for flexible authentication and access control. 
This flexibility helps consider the social relationships of users in smart homes. 
Some even call for not implementing any authentication process for people who are within proximity, as is the case for traditional home appliances. 
Others call for a dynamic design where users can have full control with facilitation to add and remove access smoothly. 
Incorporating flexibility in smart home devices by giving users more options to control is not trivial, as many research projects have not been able to balance convenience and privacy~\cite{multi-user-problem-smart-home,Too_many_Notifications}.

%\textbf{User awareness is key in preventing tech-abuse in general as well as in SHTA.}
\textbf{Smart homes call for more technical background.}
Smart homes are similar to enterprise networks more than personal computers or smartphones.
The expertise and workforce that enterprises have to manage their networks are not available for smart home users~\cite{European_Cybersecurity_report_imbalanceControlProblem}.
The case in smart homes is that some users might have more knowledge than others and this uneven power is caused by inappropriate design in the first place.

%###############################################
\begin{table*}[!t]
	\centering
	\caption{Summary of proposed solutions in the literature to combat SHOT} 
	\vspace{-9pt}
	\label{tab:techs}
	\scalebox{0.9}{%% This reduces the whole table, fonts and dimensions
	\begin{tabular}{|p{3cm}|p{0.5cm}|p{5cm}|p{4.4cm}|p{0.9cm}|p{1cm}|}
	    \hline
	    \rowcolor{Gray}
	    
		\textbf{Solution}    &  \textbf{In} &  \textbf{Downsides}&  \textbf{Objective}&  \textbf{Can victims act?}&  \textbf{Short or long term?}       \\ \hline
		
	 Involving cybersecurity experts in designing smart home devices&\cite{SmartHome_Abuse_Category_1_paper1,SmartHome_Abuse_Category_2_paper4,SmartHome_Abuse_Category_2_paper6}&   Vendors need more time and budget before launching their products.&  
	     Ensuring applicability and reliability of security features \textit{and} providing plans for front liners
	
%& Support services, vendors
&  No&  Long term       \\ \hline

 Adding labels to smart home devices similar to the nutrition labels&\cite{Security_lables}& 
      Abusers might not buy devices with safety features \textit{and} vendors need more time and budget before launching their products.
  &  
	     Raising awareness for victims \textit{and} pushing for standardizing safety in smart home devices

%& Victims, vendors
&  Yes&  Long term       \\ \hline

 Deleting usage history periodically&\cite{SmartHome_Abuse_Category_2_paper4,Stories_survivors_IPV}& 
      
          Might help abusers hide their abuse and gaslight victims~[12] \textit{and} victims might lose evidence when building a case~\cite{SmartHome_Abuse_Category_2_paper4}.
   
  &  
	     Protecting victims by hiding their escape plans
	    
%& Victims, abusers
&  Yes&  Short term       \\ \hline

Making usage history permanent  &\cite{IBM_tech_abuse_design}& 
      
          Victims struggle to hide their escape plans for victims \textit{and} personal privacy for normal users might be compromised.
       
  &  
	     Helping hold abusers accountable \textit{and} victims can have evidence when building a case~\cite{Stories_survivors_IPV,SmartHome_Abuse_Category_2_paper4}
	 
  %& Victims, abusers 
  &  No &  Short term       \\ \hline


Providing emergency access to support services to intervene in case of abuse &\cite{SmartHome_Abuse_Category_2_paper6}& 
      
          Making decisions on behalf of users is not good practice~\cite{IBM_tech_abuse_design} \textit{and} personal privacy for normal users might be compromised.
  &  
	     Helping victims reach out to support services
	      %& support services, victims 
	      &  No &  Long term       \\ \hline


Making devices distinguish users through voice recognition &
\cite{SmartHome_Abuse_Category_2_paper1,SmartHome_Abuse_Category_2_paper6}& 
      
          This leads to less controllable devices~\cite{Access_control_not_working} \textit{and} works only with voice assistants.

  &  
	     Protecting users' data from other users
	    
%& Victims, abusers 
&  No &  Long term       \\ \hline

Providing Clinical Computer Security for victims of IPV &\cite{tech-abuse-helpVictims_2}.& 
      Solution does not consider acquiring and living phases \textit{and} is hard to scale
  &  
	     Providing personalized help to victims \textit{and} keeping personnel up-to-date
	 
 %& Victims, support services 
 &  Yes &  Long term       \\ \hline

	\end{tabular}
	} %end of table scaling
	\label{literature_solutions}
	\vspace{-15pt}
\end{table*}

%##############################################

\textbf{Collecting evidence to make legal cases is hard in smart homes.}
If victims identify abuse and want to make a legal case, legal resources are limited~\cite{NY_Times_Tech_Abuse}.
Abusers exploit the excessive power they attain in most smart home devices by deleting usage histories when they gaslight their partners~\cite{SmartHome_Abuse_Category_1_paper2,IBM_tech_abuse_design}.
If abusers can not change the usage history without their partner's knowledge, this can help prevent gaslighting.
However, this same feature can be harmful when victims try to hide their awareness of abuse and their communication with support services~\cite{SmartHome_Abuse_Category_2_paper4,Stories_survivors_IPV}.


\textbf{Lack of adequate training for support services.}
Support services need up-to-date training to keep up with emerging tools that abusers use~\cite{SmartHome_Abuse_Category_2_paper4}.
Front liners are the first point of contact for victims in IPV cases. 
They always need to be equipped with the proper tools to help victims and connecting them with available resources.
The lack of expertise and training in support service providers leaves victims helpless. 


\textbf{Lack of standards and regulations that account for IPV in smart homes.}
There are no known regulations that consider SHOT that vendors can follow.
The reason behind the absence of regulations may be related to the lack of standards.
Standards by themselves can not enforce vendors to change their designs. However, standards are usually what regulations refer to when writing legislation and guidance documents~\cite{BSI_Standards_regulations}.
So if standards are created, regulations will likely be developed and enforced.
Writing standards is not trivial and requires a lot of continuous collaborations between stakeholders in the smart home industry.
Piasecki et al. review cybersecurity standards and find that they do not consider the \textit{UI-adversary} in their guidelines and recommendations~\cite{review_standards_IoT}.
In addition, IoT Security Foundation, a leading influencer in the IoT industry, surveyed the IoT industry for basic security adoptions and found that the majority of the IoT vendors were still not compliant with basic security hygiene~\cite{IoT_security_foundation}. 
This shows that the industry is still behind on basics.
Making smart home devices abuse-resistant is a step further. We do not foresee this being adopted in the near future with the current situation despite all the high risks associated with SHOT.

\iffalse
\begin{table}[!t]
	\centering
%	\caption{Summary of technical challenges in smart homes} 
	%\vspace{-10pt}
	\label{tab:techs}
	\begin{tabular}{|p{8cm}|}
		\hline
		
	%	\\ \hline
	%	\hline
	\rowcolor{Gray}
		\textbf{Summary of technical challenges in smart homes}            \\ \hline

\begin{itemize}
%    \item The blockbox nature of smart home devices is troublesome.
%    \item Recent security research did not consider \textit{UI-Adversary} in their threat models.
%    \item Smart homes call for more technical background than personal computers.
%    \item Access control in smart home devices are not reliable.
    \item Collecting evidence to make legal cases is hard in smart homes.
%    \item Smart home devices are not designed for a multi-user environment.
%    \item Lack of standards and regulations that account for IPV in smart homes.
%    \item Lack of adequate training for support services.
\end{itemize}      \\ \hline
	\end{tabular}
	\label{Table_technical_cahllenges_summary}
	%\vspace{-10pt}
\end{table}
\fi

\iffalse
\textbf{Summary of technical challenges in smart homes:}
\begin{itemize}
    \item The blockbox nature of smart home devices is troublesome.
    \item Recent security research did not consider \textit{UI-Adversary} in their threat models.
    \item Smart homes call for more technical background than personal computers.
    \item Access control in smart home devices are not reliable.
    \item Collecting evidence to make legal cases is hard in smart homes.
    \item Smart home devices are not designed for a multi-user environment.
    \item Lack of standards and regulations that account for IPV in smart homes.
    \item Lack of adequate training for support services.
\end{itemize}
\fi



Smart home technology vendors do not intentionally make their devices as tools for domestic abuse. There is in fact great evidence that smart home devices are so beneficial for several reasons such as increasing safety and saving energy.
For instance, the Los Angeles Police Department has reported that the use of Ring doorbells had reduced crimes in some of Los Angeles neighborhoods by 55 percent in seven months~\cite{Ring_Example_CrimeLess}. 
However, smart home technology vendors have not paid attention to the IPV threat. 
Lack of diversity of the design teams, poor usability of the devices, inadequate research of the IPV threat, and system malfunction or unexpected functions are the main reasons for smart home devices being an abuse vector.



%my writing below - Malek's above
\iffalse
In this section, we analyze from a technical standpoint why current smart home devices empower abusers in IPV, limit victims' abilities to protect themselves, and challenge support services to provide help.
The literature has shown that designers of smart home devices have not considered multi-user environments in the authentication mechanisms and access controls of the devices which leads to empowering abusers over victims of IPV~\cite{Access_control_not_working,European_Cybersecurity_report_imbalanceControlProblem}. 

\textbf{The blackbox nature of smart home devices is troublesome.} Litão explains how the blackbox nature of smart home devices inhibits users' abilities to understand the data flow and how this plays a big role in leading into unequal control power between intimate partners~\cite{SmartHome_Abuse_Category_2_paper1}.
The majority of smart home devices do not offer an interface on the same devices. Normally, they make use of smartphones for authentication, access control, and privacy settings~\cite{European_Cybersecurity_report_imbalanceControlProblem}. 

\textbf{Recent security research did not consider UI-Adversary in their threat models.}
Slupska conducts a thorough analysis of 44 research papers about security in smart homes and she finds that none of them has considered IPV in their threat models~\cite{feminist_Cybersecurity}.
Recent security research focused on the same security issues as in personal computers and smartphones. 
Smart homes are different from traditional technology because considering social complexities and potential unequal access is extremely important to the safety of users~\cite{European_Cybersecurity_report_imbalanceControlProblem}.

\textbf{Access control in smart home devices is not reliable.}
Janes et al. evaluate 19 popular smart home devices and find that 16 of them struggle to revoke access from previously authorized users even after changing passwords or explicitly revoking their access~\cite{Access_control_not_working}. 
This means that if abuse is identified and victims try to revoke access from their abusers, most of the smart home devices do not enforce that immediately.
This is mainly because of lengthy token expiration.
The findings in~\cite{Access_control_not_working} show that the majority of smart home devices are not reliable when victims act to protect themselves. 


\textbf{Smart home devices are not designed for a multi-user environment.}
Recent work discusses why current smart home devices are not designed for multiple users and conduct user studies to qualitatively analyze users' needs in smart homes~\cite{multi-user-problem-smart-home,Rethinking_Access_control_Authnetication}. 
The findings call for flexible authentication and access control. 
This flexibility helps considers the social relationships of users in smart homes. 
Some even call for not implementing any authentication process for people who are within proximity as is the case for traditional home appliances. 
Others call for a dynamic design where users can have full control with facilitation to add and remove access smoothly. 
Incorporating flexibility in smart home devices by giving users more options to control is not trivial as many research projects have not been able to find the right balance between convenience and privacy~\cite{multi-user-problem-smart-home,Too_many_Notifications}.

%\textbf{User awareness is key in preventing tech-abuse in general as well as in SHTA.}
\textbf{Smart homes call for more technical background.}
Smart homes are similar to enterprise networks more than personal computers or smartphones.
The expertise and workforce that enterprises have to manage their networks are not available for smart home users~\cite{European_Cybersecurity_report_imbalanceControlProblem}.
The case in smart homes is that some users might have more knowledge than others and this uneven access power is due to lack of appropriate design in the first place.

%###############################################
\begin{table*}[!t]
	\centering
	\caption{Summary of proposed solutions in the literature to combat SHOT} 
	\vspace{-9pt}
	\label{tab:techs}
	\scalebox{0.9}{%% This reduces the whole table, fonts and dimensions
	\begin{tabular}{|p{3cm}|p{0.5cm}|p{5cm}|p{4.4cm}|p{0.9cm}|p{1cm}|}
	    \hline
	    \rowcolor{Gray}
	    
		\textbf{Solution}    &  \textbf{In} &  \textbf{Conflicts and downsides}&  \textbf{Goal}&  \textbf{Victims can act}&  \textbf{Short or long term}       \\ \hline
		
	 Involving cybersecurity experts in designing smart home devices&\cite{SmartHome_Abuse_Category_1_paper1,SmartHome_Abuse_Category_2_paper4,SmartHome_Abuse_Category_2_paper6}&   Vendors need more time and budget before launching their products&  
	     Ensuring applicability and reliability of security features \textit{and} providing plans for front liners
	
%& Support services, vendors
&  No&  Long term       \\ \hline

 Adding labels to smart home devices similar to the nutrition labels&\cite{Security_lables}& 
      Abusers might not buy devices with safety features, \textit{and} vendors need more time and budget before launching their products
  &  
	     Raising awareness for victims \textit{and} pushing for standardizing safety in smart home devices

%& Victims, vendors
&  Yes&  Long term       \\ \hline

 Deleting usage history periodically&\cite{SmartHome_Abuse_Category_2_paper4,Stories_survivors_IPV}& 
      
          This might help abusers hide their abuse and gaslight victims~\cite{SmartHome_Abuse_Category_2_paper3}, \textit{and} victims might lose evidence when building a case~\cite{SmartHome_Abuse_Category_2_paper4}
   
  &  
	     Protecting victims by hiding their escape plans
	    
%& Victims, abusers
&  Yes&  Short term       \\ \hline

Making usage history permanent  &\cite{IBM_tech_abuse_design}& 
      
          Victims struggle to hide their escape plans, \textit{and} personal privacy for normal users might be compromised
       
  &  
	     Helping hold abusers accountable \textit{and} victims can have evidence when building a case~\cite{Stories_survivors_IPV,SmartHome_Abuse_Category_2_paper4}
	 
  %& Victims, abusers 
  &  No &  Short term       \\ \hline


Including access for support services to intervene in case of abuse &\cite{SmartHome_Abuse_Category_2_paper6}& 
      
          Making decisions on behalf of users is not good practice~\cite{IBM_tech_abuse_design} \textit{and} personal privacy for normal users might be compromised
  &  
	     Helping victims reach out to support services
	      %& support services, victims 
	      &  No &  Long term       \\ \hline


Making devices differentiate multi-user by voice recognition &
\cite{SmartHome_Abuse_Category_2_paper1,SmartHome_Abuse_Category_2_paper6}& 
      
          Less controllable devices~\cite{Access_control_not_working} \textit{and} this works only for voice assistants

  &  
	     Protecting users' data from other users
	    
%& Victims, abusers 
&  No &  Long term       \\ \hline

Providing Clinical Computer Security for victims of IPV &\cite{tech-abuse-helpVictims_2}& 
      Does not consider acquiring and living phases \textit{and} it is hard to scale
  &  
	     Providing personalized help to victims \textit{and} keeping IPV personnel up-to-date
	 
 %& Victims, support services 
 &  Yes &  Long term       \\ \hline

	\end{tabular}
	} %end of table scaling
	\label{literature_solutions}
	\vspace{-15pt}
\end{table*}

%##############################################

\textbf{Collecting evidence to make legal cases is hard in smart homes.}
If victims identify abuse and want to make a legal case, legal resources are limited~\cite{NY_Times_Tech_Abuse}.
Abusers exploit the excessive power they attain in most smart home devices by deleting usage histories when they gaslight their partners~\cite{SmartHome_Abuse_Category_1_paper2,IBM_tech_abuse_design}.
If abusers can not change the usage history without their partner's knowledge, this can help prevent gaslighting.
However, this same feature can be harmful when victims try to hide their awareness of abuse and their contacts with support services~\cite{SmartHome_Abuse_Category_2_paper4,Stories_survivors_IPV}.


\textbf{Lack of adequate training for support services.}
Support services need up-to-date training to keep up with emerging tools that abusers use~\cite{SmartHome_Abuse_Category_2_paper4}.
Front liners are the first point of communication for victims in IPV cases. 
They always need to be equipped with the proper tools to provide help to victims and start contacting with available resources.
The lack of expertise and training in support services leaves victims helpless. 


\textbf{Lack of standards and regulations that account for IPV in smart homes.}
There are no known regulations that consider SHOT so corresponding vendors can follow.
The reason behind the absence of regulations can be related to the absence of standards.
Standards by themselves can not enforce vendors to change their designs. However, standards are usually what regulations refer to when writing legislation and guidance documents~\cite{BSI_Standards_regulations}.
Thus, if standards are created, regulations will likely be written and enforced.
Writing standards is not trivial and requires a lot of continuous collaborations between stakeholders in the smart home industry.
Piasecki et al. review cybersecurity standards and find that they do not consider the \textit{UI-adversary} in their guidelines and recommendations~\cite{review_standards_IoT}.
In addition, IoT Security Foundation, which is a leading influencer in the IoT industry, surveys the IoT industry for basic security adoptions and finds that the majority of the IoT vendors are still not compliant with basic security hygiene~\cite{IoT_security_foundation}. 
This tells us that the industry is still behind on basics.
Making smart home devices abuse-resistant is a step further and we do not foresee this being adopted in the near future with the current situation despite the high risks associated with SHOT.

\iffalse
\begin{table}[!t]
	\centering
%	\caption{Summary of technical challenges in smart homes} 
	%\vspace{-10pt}
	\label{tab:techs}
	\begin{tabular}{|p{8cm}|}
		\hline
		
	%	\\ \hline
	%	\hline
	\rowcolor{Gray}
		\textbf{Summary of technical challenges in smart homes}            \\ \hline

\begin{itemize}
%    \item The blockbox nature of smart home devices is troublesome.
%    \item Recent security research did not consider \textit{UI-Adversary} in their threat models.
%    \item Smart homes call for more technical background than personal computers.
%    \item Access control in smart home devices are not reliable.
    \item Collecting evidence to make legal cases is hard in smart homes.
%    \item Smart home devices are not designed for a multi-user environment.
%    \item Lack of standards and regulations that account for IPV in smart homes.
%    \item Lack of adequate training for support services.
\end{itemize}      \\ \hline
	\end{tabular}
	\label{Table_technical_cahllenges_summary}
	%\vspace{-10pt}
\end{table}
\fi

\iffalse
\textbf{Summary of technical challenges in smart homes:}
\begin{itemize}
    \item The blockbox nature of smart home devices is troublesome.
    \item Recent security research did not consider \textit{UI-Adversary} in their threat models.
    \item Smart homes call for more technical background than personal computers.
    \item Access control in smart home devices are not reliable.
    \item Collecting evidence to make legal cases is hard in smart homes.
    \item Smart home devices are not designed for a multi-user environment.
    \item Lack of standards and regulations that account for IPV in smart homes.
    \item Lack of adequate training for support services.
\end{itemize}
\fi



Smart home technology vendors do not intentionally make their devices as tools for domestic abuse. There is in fact great evidence that smart home devices are so beneficial for several reasons such as increasing safety and saving energy.
For instance, the Los Angeles Police Department has reported that the use of Ring doorbells had reduced crimes in some of Los Angeles neighborhoods by 55 percent in seven months~\cite{Ring_Example_CrimeLess}. 
However, smart home technology vendors have not paid attention to the threat arising in IPV. 
Lack of diversity in the designing teams, poor usability of the devices, inadequate research of the threat of IPV in smart homes, and system functions do not work as expected are the main reasons for smart home devices being not abuse-resistant.


\fi

==> Tech-abuse_SmartHomes_Draft 2-3/TexFiles/abstract.tex <==
Smart home devices have brought us many benefits such as advanced security, convenience, and entertainment. However, these devices also have made unintended consequences like giving ultimate power for devices' owners over their intimate partners in the same household which might lead to tech-facilitated domestic abuse (tech-abuse) as recent research has shown. 
In this paper, we systematize findings on tech-abuse in smart homes.
We show that domestic abuse and Intimate Partner Violence (IPV) in smart homes is more effective and less risky for abusers. Victims find it more harmful and more challenging to protect themselves from.
We articulate a comprehensive analysis of all the phases of abuse in smart homes and categorize risks and needs in each phase. 
Technical analysis of current smart home technologies is conducted to shed light upon their limitations.
%\hl{Key insights resulting from works both in the IPV and smart home communities are identified and the effectiveness of approaches are related to tech-abuse in smart homes.}
%We then survey the literature to analyze all the phases of abuse and explain in detail the promising findings and their shortcomings.
We also summarize recent recommendations to combat tech-abuse in smart homes and focus on their  potentials and shortcomings.
Unsurprisingly, we find that many recommendations conflict with each other due to a lack of understanding of phases of abuse in smart homes.
%In the end, we provide several 
Desirable properties to design abuse-resistant smart home devices are proposed for all the phases of abuse.
The research community benefits from our analysis and recommendations to move forward with a focus on filling the blind spots of existing smart home devices' safety measures and building appropriate safety measures that consider tech-abuse threats in smart homes.

\iffalse

Smart home devices have brought us many benefits such as advanced security, convenience, and entertainment. However, these devices also have made unintended consequences like giving ultimate power for devices' owners over their intimate partners in the same household which might lead to tech-facilitated domestic abuse (tech-abuse) as recent research has shown. 
In this paper, we systematize findings on tech-abuse in smart homes.
We show that domestic abuse and Intimate Partner Violence (IPV) in smart homes is more effective and less risky for abusers. Victims find it more harmful and more challenging to protect themselves from.
We articulate a comprehensive analysis of all the phases of abuse in smart homes and categorize risks and needs in each phase. 
Technical analysis of current smart home technologies is conducted to shed light upon their limitations.
%\hl{Key insights resulting from works both in the IPV and smart home communities are identified and the effectiveness of approaches are related to tech-abuse in smart homes.}
%We then survey the literature to analyze all the phases of abuse and explain in detail the promising findings and their shortcomings.
We also summarize recent recommendations to combat tech-abuse in smart homes and focus on their  potentials and shortcomings.
Unsurprisingly, we find that many recommendations conflict with each other due to a lack of understanding of phases of abuse in smart homes.
%In the end, we provide several 
Desirable properties to design abuse-resistant smart home devices are proposed for all the phases of abuse.
The research community benefits from our analysis and recommendations to move forward with a focus on filling the blind spots of existing smart home devices' safety measures and building appropriate safety measures that consider tech-abuse threats in smart homes.
\fi

==> Tech-abuse_SmartHomes_Draft 2-3/TexFiles/background.tex <==
\subsection{Background}

%     Some traditional abuse techniques
%    \newline Some defenses techniques
%    \newline Some regulations and support services to combat traditional abuse
%    \newline Idea: give short names to all different abuse types to prevent ambiguity throughout the paper. For example, traditional abuse, tech-based abuse and smart home-facilitated tech-abuse (SMTA).

\iffalse
\subsubsection{Smart homes}
Smart homes consist of Internet of Things (IoT) devices that can sense ambient environments such as smart lighting, smart thermostat, and indoor cameras, and transform physical readings into digital data to be dealt with by processors.
The common characteristics among smart home devices are their ability to connect to the Internet and being able to sense or change the ambiance.
In this paper, we refer to smart homes as a house with one or more smart home devices. 
\fi
%\subsubsection{Domestic abuse}
According to the United States Department of Justice Office on Violence Against Women, domestic violence is a pattern of abusive behavior in any relationship that is used by one partner to gain or maintain control over another intimate partner~\cite{DoJ_OVW_Domestic_Definition}. 
There are three types of abuse: 
\begin{itemize}
	\item \textbf{Traditional abuse}: Any abusive actions that do not use technology, 
	\item \textbf{Tech-abuse}: Any abusive actions using technologies such as smartphones, personal computers, or social media websites, and 
	\item \textbf{Tech-abuse in smart homes}: Any abusive actions that use smart home devices. 
\end{itemize}

To prevent ambiguity, we refer to tech-abuse in smart homes as Smart HOme facilitated Tech-abuse (\textit{\textbf{SHOT}}).

%Many types of abuse are included in the definition of domestic violence such as physical, emotional, psychological abuse, or others~\cite{DoJ_OVW_Domestic_Definition}. 

\iffalse
\begin{itemize}
    \item Traditional abuse: any abusive actions that do not use technology.
    \item Tech-abuse: any abusive actions using technologies that have been used for more than ten years such as smartphones, personal computers, or social media websites.
    Tech-abuse in this paper refers to this kind of tech-abuse.
    \item Tech-abuse in smart homes: any abusive actions that use smart home devices. To prevent ambiguity, we refer to this kind of abuse as Smart Home facilitated Tech-Abuse (SHTA).
\end{itemize}
In this paper, we focus on tech-abuse using smart home devices (SHTA).
\fi

\iffalse % To comment out multiple lines
\subsubsection{Stakeholders in IPV}
Domestic abuse involves more than the abuser and the victim.
In many countries, support services exist for victims in case of domestic abuse.
These services offer help in many ways such as talking with specialists, getting therapy, and building a legal case with attorneys. 
Below we define all the entities involved in IPV cases:
\begin{itemize}
\item The abuser: the person who uses any form of violence to hurt his/her intimate partner.
\item The victim: the person who might be affected by the abuser.
\item Support services: governmental or charitable organizations that provide services to help stop abusers and support victims. 
These services include organizations, law enforcement, courts
\end{itemize}
\fi


%\subsection{Related work}

%%#####
%We can change related work to include 3 projects
%Clinical Computer Security for Victims of Intimate Partner Violence
% Towards a holistic ICT platform for protecting intimate partner violence survivors based on the IoT paradigm
% IBM design principles
\iffalse
There has been a noticeable effort by researchers to combat tech-abuse in general. 
For instance, researchers have analyzed tech-abuse in social media where abusers can stalk, impersonate, or harass their intimate partners on social media websites like Facebook or Twitter~\cite{social_media_IPV}. 
Another example is the use of smartphones or personal computers by abusers to harm their intimate partners~\cite{tech-abuse-helpVictims_1}. 
\hl{Both of these examples are different than tech-abuse in smart home environments.
Stalking users in smart homes is a day long without the need for any users' interactions in many cases while stalking in smartphones or social media is only effective when there is a user's interaction.}
\fi
Many recent research projects on domestic abuse in smart homes were user studies. The studies qualitatively analyze victim's needs in smart homes or front-liners' needs of support services to combat abusers in IPV~\cite{SmartHome_Abuse_Category_1_paper1,SmartHome_Abuse_Category_2_paper1, SmartHome_Abuse_Category_2_paper2, SmartHome_Abuse_Category_1_paper2}. 
Other researchers partially considered SHOT without analyzing its corresponding specific abuse phases.
Havron et al. propose a solution similar to a medical clinic, where an IPV victim can reach out to support services and an expert can provide personalized help~\cite{tech-abuse-helpVictims_2}.
Kotz et al. discuss unique challenges in ensuring human safety in smart environments and encourage designers to consider these challenges while developing products~\cite{challenges_safety_smart_Environments}.
Nuttall et al. propose five design principles that vendors should consider when developing new technologies to prevent coercive control for abusers~\cite{IBM_tech_abuse_design}. 
These research efforts focus on tech-abuse generally and we argue that tech-abuse in smart homes is unique and calls for specific considerations.
In short, there has not been a thorough analysis of specific phases of abuse in smart homes, technical reasons for empowering abusers, and concrete breakdowns of security and safety issues of SHOT.
Safety in this paper means that smart home security and privacy measures fail and personal safety of users becomes at risk.

%The main focus is on the lifecycle of IoT devices in general.
%Also, IoT devices can be deployed in many environments such as smart offices, smart hotels, or smart cities.
%However, we focus on phases of tech-abuse in smart homes which is more specific, and we consider phases of abuse which is not the case in~\cite{challenges_safety_smart_Environments}.

\iffalse To the best of our understanding, we are the first to explore tech-abuse in smart homes from a wider perspective considering all phases of abuse and break down the security and privacy issues for each phase.
In addition, literature in tech-abuse has not explored the problems of victims' ability to recognize abuse and needs when acquiring new smart home devices.
Thus, we add two new phases to the traditional phases that cover missing phases in the literature.
In Section \ref{phases}, we cover the literature of SHOT in detail concerning the phases of abuse.
\fi





%Rodríguez-Rodríguez et al. have analyzed the literature of IPV using IoT technologies~\cite{Home_Abuse_Category_2_paper6}. Authors focus on the solutions provided by previous research and categorize them. The difference between their work and ours is that we analyze the IPV in smart home specifically and look at the other stakeholders such as research in IPV




\subsection{Differences between Tech-abuse and SHOT}
Tech-based abuse is when abusers use technology such as smartphones or computers to carry out harmful actions to their partners. 
There are similar characteristics of this kind of abuse. 
Devices are owned by the victim but might be accessed by the abuser.
Threats lie around what the victim might do in their gadgets such as calls made, posts on social media, or usage of some apps. 
The research community has reasonably offered Privacy Enhancing Technologies (PET) to victims to protect themselves~\cite{tech-abuse-helpVictims_1,tech-abuse-helpVictims_2}. 
In short, smartphones and personal computers have been the subject of research in tech-abuse. This has led to many defense mechanisms. 
\begin{figure*}[t]
\centerline{
\includegraphics[scale=.5]{./Figures/Phases_Framework_Resized_July21.pdf}}
\vspace{-0.4cm}
\caption{Our framework of phases of SHOT with the corresponding goals for each entity involved.}
\label{phases_figure}
\vspace{-17pt}
\end{figure*}


Nevertheless, tech-abuse in smart homes (SHOT) is relatively new. 
This calls for more research to explore the technical and social complexities as well as the design issues. 
Abusers' abilities to harm their intimate partners have advanced greatly with smart home devices. Abusers can now use effective, efficient, and untraceable methods to carry out stalking, gaslighting, and other abusive actions~\cite{SmartHome_Abuse_Category_1_paper1}. 
Also, devices in smart homes are not necessarily owned by victims. Rather, they are largely owned and controlled by abusers~\cite{SmartHome_Abuse_Category_1_paper2}. 
These devices can modify the ambient environment and unlock the door of the house. 
Simply, they can impact the physical surroundings which is more damaging than just dealing with digital data. 
%A good example to explain the difference between tech-abuse using smartphones and smart homes is that a laptop is shared between family members with the browsing history being visible to everyone. 
%Imagine if the browsing history is not only about what websites you have visited, it is about what you have done in the house.
%In addition to the breach of privacy that could happen in smart homes, the devices could be actuated to change ambient environments, lock status, and indoor footage. 



Table \ref{abuse_comparison} demonstrates the differences between the three types of abuse. We consider three metrics to evaluate the abuse methods: the required effort to carry out the abuse, the risk taken by abusers, and the benefit to the abusers.
Estimating effort takes into account the time spent carrying out the abuse, the proximity of the abuser to the victim, and the speed of the action (whether immediate or not).
Risk is approximately measured by how victims can defend themselves which will impact abusers and hold them accountable.
In the formal definition of domestic abuse, abusers seek to control their intimate partners for a variety of reasons.
In Table  \ref{abuse_comparison}, we estimate the benefits to abusers by looking at how much control they can attain through the tools used in all the three methods of abuse to perform abusive actions.
The stalking example in Table \ref{abuse_comparison} shows that tech-abuse using smart home devices calls for less effort, lower risk, and more rewards for abusers. 
This makes exploiting smart home devices for abusers in IPV an ideal tool to carry out their harmful activities. 
%In Section \ref{phases}, we show the current state of research in IPV in smart homes, and the corresponding solutions to prevent empowering abusers, empower victims, and assist support services.


\iffalse % my writing is below as a whole - Malek's edit is above

\subsection{Background}


%my writing below


\iffalse
\subsubsection{Smart homes}
Smart homes consist of Internet of Things (IoT) devices that can sense ambient environments such as smart lighting, smart thermostat, and indoor cameras, and transform physical readings into digital data to be dealt with by processors.
The common characteristics among smart home devices are their ability to connect to the Internet and being able to sense or change the ambiance.
In this paper, we refer to smart homes as a house with one or more smart home devices. 
\fi
%\subsubsection{Domestic abuse}
According to the United States Department of Justice Office on Violence Against Women, domestic violence is a pattern of abusive behavior in any relationship that is used by one partner to gain or maintain control over another intimate partner~\cite{DoJ_OVW_Domestic_Definition}. 
There are three types of abuse: 
\iffalse
\textbf{traditional abuse} which is any abusive actions that do not use technology, \textbf{tech-abuse} which is any abusive actions using technologies such as smartphones, personal computers, or social media websites, and \textbf{tech-abuse in smart homes} which is any abusive actions that use smart home devices. To prevent ambiguity, we refer to tech-abuse in smart homes as Smart HOme facilitated Tech-abuse (\textit{\textbf{SHOT}}).
\fi
%\iffalse
\begin{itemize}
	\item \textbf{Traditional abuse}: Any abusive actions that do not use technology, 
	\item \textbf{Tech-abuse}: Any abusive actions using technologies such as smartphones, personal computers, or social media websites, and 
	\item \textbf{Tech-abuse in smart homes}: Any abusive actions that use smart home devices. 
\end{itemize}

To prevent ambiguity, we refer to tech-abuse in smart homes as Smart HOme facilitated Tech-abuse (\textit{\textbf{SHOT}}).
%\fi

%Many types of abuse are included in the definition of domestic violence such as physical, emotional, psychological abuse, or others~\cite{DoJ_OVW_Domestic_Definition}. 

\iffalse
\begin{itemize}
    \item Traditional abuse: any abusive actions that do not use technology.
    \item Tech-abuse: any abusive actions using technologies that have been used for more than ten years such as smartphones, personal computers, or social media websites.
    Tech-abuse in this paper refers to this kind of tech-abuse.
    \item Tech-abuse in smart homes: any abusive actions that use smart home devices. To prevent ambiguity, we refer to this kind of abuse as Smart Home facilitated Tech-Abuse (SHTA).
\end{itemize}
In this paper, we focus on tech-abuse using smart home devices (SHTA).
\fi

\iffalse % To comment out multiple lines
\subsubsection{Stakeholders in IPV}
Domestic abuse involves more than the abuser and the victim.
In many countries, support services exist for victims in case of domestic abuse.
These services offer help in many ways such as talking with specialists, getting therapy, and building a legal case with attorneys. 
Below we define all the entities involved in IPV cases:
\begin{itemize}
\item The abuser: the person who uses any form of violence to hurt his/her intimate partner.
\item The victim: the person who might be affected by the abuser.
\item Support services: governmental or charitable organizations that provide services to help stop abusers and support victims. 
These services include organizations, law enforcement, courts
\end{itemize}
\fi


%\subsection{Related work}

%%#####
%We can change related work to include 3 projects
%Clinical Computer Security for Victims of Intimate Partner Violence
% Towards a holistic ICT platform for protecting intimate partner violence survivors based on the IoT paradigm
% IBM design principles
\iffalse
There has been a noticeable effort by researchers to combat tech-abuse in general. 
For instance, researchers have analyzed tech-abuse in social media where abusers can stalk, impersonate, or harass their intimate partners on social media websites like Facebook or Twitter~\cite{social_media_IPV}. 
Another example is the use of smartphones or personal computers by abusers to harm their intimate partners~\cite{tech-abuse-helpVictims_1}. 
\hl{Both of these examples are different than tech-abuse in smart home environments.
Stalking users in smart homes is a day long without the need for any users' interactions in many cases while stalking in smartphones or social media is only effective when there is a user's interaction.}
\fi
Many recent research projects on domestic abuse in smart homes were user studies. The studies qualitatively analyze victim's needs in smart homes or front-liners' needs of support services to combat abusers in IPV~\cite{SmartHome_Abuse_Category_1_paper1,SmartHome_Abuse_Category_2_paper1, SmartHome_Abuse_Category_2_paper2, SmartHome_Abuse_Category_1_paper2}. 
Other researchers partially considered SHOT without analyzing its corresponding specific abuse phases.
Havron et al. propose a solution similar to a medical clinic, where an IPV victim can reach out to support services and an expert can provide personalized help~\cite{tech-abuse-helpVictims_2}.
Kotz et al. discuss unique challenges in ensuring human safety in smart environments and encourage designers to consider these challenges while developing products~\cite{challenges_safety_smart_Environments}.
Nuttall et al. propose five design principles that vendors should consider when developing new technologies to prevent coercive control for abusers~\cite{IBM_tech_abuse_design}. 
These research efforts focus on tech-abuse generally and we argue that tech-abuse in smart homes is unique and calls for specific considerations.
In short, there has not been a thorough analysis of specific phases of abuse in smart homes, technical reasons for empowering abusers, and concrete breakdowns of security and safety issues of SHOT.
Safety in this paper means that smart home security and privacy measures fail and personal safety of users becomes at risk.

%The main focus is on the lifecycle of IoT devices in general.
%Also, IoT devices can be deployed in many environments such as smart offices, smart hotels, or smart cities.
%However, we focus on phases of tech-abuse in smart homes which is more specific, and we consider phases of abuse which is not the case in~\cite{challenges_safety_smart_Environments}.

\iffalse To the best of our understanding, we are the first to explore tech-abuse in smart homes from a wider perspective considering all phases of abuse and break down the security and privacy issues for each phase.
In addition, literature in tech-abuse has not explored the problems of victims' ability to recognize abuse and needs when acquiring new smart home devices.
Thus, we add two new phases to the traditional phases that cover missing phases in the literature.
In Section \ref{phases}, we cover the literature of SHOT in detail concerning the phases of abuse.
\fi





%Rodríguez-Rodríguez et al. have analyzed the literature of IPV using IoT technologies~\cite{Home_Abuse_Category_2_paper6}. Authors focus on the solutions provided by previous research and categorize them. The difference between their work and ours is that we analyze the IPV in smart home specifically and look at the other stakeholders such as research in IPV




\subsection{Differences between Tech-abuse and SHOT}
Tech-based abuse is when abusers use technology such as smartphones or computers to carry out harmful actions to their partners. 
There are similar characteristics of this kind of abuse. 
Devices are owned by the victim but might be accessed by the abuser.
Threats lie around what the victim might do in their gadgets such as calls made, posts on social media, or usage of some apps. 
The research community has reasonably offered Privacy Enhancing Technologies (PET) to victims to protect themselves~\cite{tech-abuse-helpVictims_1,tech-abuse-helpVictims_2}. 
In short, smartphones and personal computers have been the subject of research in tech-abuse. This has led to many defense mechanisms. 
\begin{figure*}[t]
\centerline{
\includegraphics[scale=.5]{./Figures/Phases_Framework_Resized_July21.pdf}}
\vspace{-0.4cm}
\caption{Our framework of phases of SHOT with the corresponding goals for each entity involved.}
\label{phases_figure}
\vspace{-17pt}
\end{figure*}


Nevertheless, tech-abuse in smart homes (SHOT) is relatively new. 
This calls for more research to explore the technical and social complexities as well as the design issues. 
Abusers' abilities to harm their intimate partners have advanced greatly with smart home devices. Abusers can now use effective, efficient, and untraceable methods to carry out stalking, gaslighting, and other abusive actions~\cite{SmartHome_Abuse_Category_1_paper1}. 
Also, devices in smart homes are not necessarily owned by victims. Rather, they are largely owned and controlled by abusers~\cite{SmartHome_Abuse_Category_1_paper2}. 
These devices can modify the ambient environment and unlock the door of the house. 
Simply, they can impact the physical surroundings which is more damaging than just dealing with digital data. 
%A good example to explain the difference between tech-abuse using smartphones and smart homes is that a laptop is shared between family members with the browsing history being visible to everyone. 
%Imagine if the browsing history is not only about what websites you have visited, it is about what you have done in the house.
%In addition to the breach of privacy that could happen in smart homes, the devices could be actuated to change ambient environments, lock status, and indoor footage. 



Table \ref{abuse_comparison} demonstrates the differences between the three types of abuse. We consider three metrics to evaluate the abuse methods: the required effort to carry out the abuse, the risk taken by abusers, and the benefit to the abusers.
Estimating effort takes into account the time spent carrying out the abuse, the proximity of the abuser to the victim, and the speed of the action (whether immediate or not).
Risk is approximately measured by how victims can defend themselves which will impact abusers and hold them accountable.
In the formal definition of domestic abuse, abusers seek to control their intimate partners for a variety of reasons.
In Table  \ref{abuse_comparison}, we estimate the benefits to abusers by looking at how much control they can attain through the tools used in all the three methods of abuse to perform abusive actions.
The stalking example in Table \ref{abuse_comparison} shows that tech-abuse using smart home devices calls for less effort, lower risk, and more rewards for abusers. 
This makes exploiting smart home devices for abusers in IPV an ideal tool to carry out their harmful activities. 
%In Section \ref{phases}, we show the current state of research in IPV in smart homes, and the corresponding solutions to prevent empowering abusers, empower victims, and assist support services.
\fi

==> Tech-abuse_SmartHomes_Draft 2-3/TexFiles/threatModel.tex <==
%Smart home devices are normally designed for homes where trust is established without any dispute.
%However, this is not realistic as IPV cases are common globally.
%The 2019 report of homicide by the United Nations (UN) has shown that one in three women has been killed by their partners~\cite{UN_Report_homicide}.
%The same report shows that two in three women are more likely to be killed at their home by a relative.

The default trust assumption in homes is problematic and could be abused by intimate partners. 
We assume devices and networks in smart homes are secure from device malfunctions, software bugs, or being compromised with the current security measures. 
Our threat model lies when authenticated users are legitimate, but with ill intentions to abuse devices' features to harm their intimate partners. 
Freed et al. refer to this threat model as UI-bound adversary~\cite{SmartHome_Abuse_Category_1_paper2}.
%We consider all forms of domestic abuse like eavesdropping, gaslighting, and others~\cite{NDVH_abuse_signs}.
%A lot of security measures try to strengthen the authentication mechanisms like implementing a two-factor authentication approach or access control of smart home devices by considering contexts of requests~\cite{softAuthZ_ContextAware}. 
%However, these measures do not normally cover the threat presented in IPV environments. 
Attackers (abusers) do not need to be sophisticated, nor delusional. 
%For example, abusers do not need programming skills nor privilege escalation.
They simply use features of the smart home devices legitimately (but maliciously) to carry out abusive actions without the need for programming skills or privilege escalation.
%There is another threat model arising from the fact that smart home devices do not do well in terms of revoking access as shown in […]. Compared to the first threat model, 


%The red background for  the acting phase represents the danger that comes from the fact that abusers will escalate their aggressiveness to not lose control of their victims~\cite{SmartHome_Abuse_Category_2_paper4}. The green background for the living phase represents that victims are in the safest stage relatively to other phases.

\iffalse

%Smart home devices are normally designed for homes where trust is established without any dispute.
%However, this is not realistic as IPV cases are common globally.
%The 2019 report of homicide by the United Nations (UN) has shown that one in three women has been killed by their partners~\cite{UN_Report_homicide}.
%The same report shows that two in three women are more likely to be killed at their home by a relative.

The default trust assumption in homes is problematic and could be abused by intimate partners. 
We assume devices and networks in smart homes are secure from device malfunctions, software bugs, or being compromised with the current security measures. 
Our threat model lies when authenticated users are legitimate, but with ill intentions to abuse devices' features to harm their intimate partners. 
Freed et al. refer to this threat model as UI-bound adversary~\cite{SmartHome_Abuse_Category_1_paper2}.
%We consider all forms of domestic abuse like eavesdropping, gaslighting, and others~\cite{NDVH_abuse_signs}.
%A lot of security measures try to strengthen the authentication mechanisms like implementing a two-factor authentication approach or access control of smart home devices by considering contexts of requests~\cite{softAuthZ_ContextAware}. 
%However, these measures do not normally cover the threat presented in IPV environments. 
Attackers (abusers) do not need to be sophisticated, nor delusional. 
%For example, abusers do not need programming skills nor privilege escalation.
They simply use features of the smart home devices legitimately (but maliciously) to carry out abusive actions without the need for programming skills or privilege escalation.
%There is another threat model arising from the fact that smart home devices do not do well in terms of revoking access as shown in […]. Compared to the first threat model, 


%The red background for  the acting phase represents the danger that comes from the fact that abusers will escalate their aggressiveness to not lose control of their victims~\cite{SmartHome_Abuse_Category_2_paper4}. The green background for the living phase represents that victims are in the safest stage relatively to other phases.
\fi

==> Tech-abuse_SmartHomes_Draft 2-3/tools/README <==

August 26, 2015


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.

 2. The \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later.

 3. The \IEEEnoauxwrite command.

 4. The IEEE itemize, enumerate and description list environments.

 5. The complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

 6. The \IEEEQEDhere and \IEEEQEDhereams commands to provide amsthm.sty
    \qedhere functionality to IEEEproof. \IEEEQEDhere is for simple use
    "right on the spot" such as within an IEEEeqnarry:

    \begin{IEEEproof}
       \begin{IEEEeqnarray}{rCl+x*}
        x & = & y & \nonumber\IEEEQEDhere
       \end{IEEEeqnarray}
    \end{IEEEproof}

    While \IEEEQEDhereams is like amsthm's venerable \qedhere and is
    for use within the standard equation environment:

    \begin{IEEEproof}
     \begin{equation}
       x = y \nonumber\IEEEQEDhereams\quad
     \end{equation}
    \end{IEEEproof}

    Note that the qedhere style is normally not done with IEEE-related
    work so these are undocumented features of IEEEtran.cls.

    Thanks Mark D. Butala, Hennadiy Leontyev and Stefan M. Moser for
    suggesting this feature.



IEEEtrantools.sty is not needed and should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
2015/08/26 V1.5 (V1.8b of IEEEtran.cls) changes:

 1) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 2) Fix bug with IEEEeqnarray equation number foreground color
    under the color environment of Beamer class.
    Thanks to Joschi Brauchle for reporting this problem.

 3) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.



********************************** Files **********************************

README                - This file.

changelog.txt         - The revision history.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> TexFiles/Discussion.tex <==
\begin{itemize}
    \item Shortcomings and challenges
    \begin{itemize}
        \item Challenges: privacy might be violated if we add adds-on features by hackers.
        \item Technology-enabled abuse leads to fear of technology.This might hurt the industry if consumers lose trust in the products...
        \item IFTTT and trigger-action platforms challenge and opportunities.
        \item What we’ve seen time and time again is that perpetrators tend to be one step ahead in leveraging technology to use it as a tool for abuse~\cite{Wired-smartHomes_abuse}.
        \item abusers might take advantage of safety labels by not buying devices with safety features. In order to make safety labels work, legislature needs to enforce all smart home vendors include safety features and labels.
    \end{itemize}
     
    How to balance between privacy and safety.
    \item Our recommendations
    \begin{itemize}
        \item For vendors
        \begin{itemize}
            \item Adversarial training in form of abuse. So that devices can be resilient to being abused.
            \item If vendors are unable for any reason to provide abuse-resistant devices, they should at least provide guidelines for support services in case of domestic abuse cases. So, when a victim of IPV reaches out to the support services, the victim will be provided with actionable advice. 
        \end{itemize}
        \item For support services. Corona Virus Disease (\textit{aka} COVID-19) crisis has been devastating in many ways. People have lost their loved ones, their jobs and other suffered an increase in the frequency and severity of domestic abuse. The number of reported domestic abuse has been skyrocketing as shown in recent articles~\cite{DomesticAbuse_Rise_COVID}. 
        \item For law enforcement and legislators: require owners to disclose other users in the house.
        \item For users
    \end{itemize}
\end{itemize}


There have not been projects that directly focus on domestic abuse in smart homes with respect to the phases of abuse, and break down the security and privacy issues to make them easier to tackle for smart home device developers.
However, there has been noticeable efforts on similar issues.
For instance, some privacy issues arise in nursing homes when residents' families suspect mistreatment from caregivers so that they set up indoor cameras~\cite{nursing_homes_privacy}. 
This act complicates the process of data collections and violation of some stakeholders' privacy. 
States like Arizona have produced bills to regulate the use of smart devices in nursing homes.
However, there is a lack of regulations in tech-abuse, let alone SHTA. 
%This is similar to our project from the perspective of 



\subsection{Limitations}
\input{TexFiles/Limitation}

\begin{table}[!t]
	\centering
	\caption{Summary of literature for tech-abuse using smart home devices- \textit{to be edited}} 
	%\vspace{-10pt}
	\label{tab:techs}
	\begin{tabular}{|l|l|}
		\hline
		\rowcolor{Gray}
		\textbf{Focus}    &  \textbf{Tech-abuse in smart homes}        \\ \hline
	    Abuser in IPV     & \cite{SmartHome_Abuse_Category_1_paper1,SmartHome_Abuse_Category_1_paper2,SmartHome_Abuse_Category_3_paper1}   \\ \hline
		Victims in IPV & \cite{SmartHome_Abuse_Category_2_paper1,SmartHome_Abuse_Category_2_paper2,SmartHome_Abuse_Category_2_paper3,SmartHome_Abuse_Category_2_paper4,SmartHome_Abuse_Category_2_paper5,homeGuard_abuse_recognize_seekHelp,SmartHome_Abuse_Category_2_paper6}    \\ \hline
		Support services for IPV victims   & \cite{SmartHome_Abuse_Category_1_paper1,SmartHome_Abuse_Category_3_paper1,homeGuard_abuse_recognize_seekHelp}    \\ \hline
	\end{tabular}
	\label{TA_features}
	%\vspace{-10pt}
\end{table}


==> TexFiles/Limitation.tex <==
Limitations and future work.

==> tools/README <==

August 26, 2015


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.

 2. The \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later.

 3. The \IEEEnoauxwrite command.

 4. The IEEE itemize, enumerate and description list environments.

 5. The complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

 6. The \IEEEQEDhere and \IEEEQEDhereams commands to provide amsthm.sty
    \qedhere functionality to IEEEproof. \IEEEQEDhere is for simple use
    "right on the spot" such as within an IEEEeqnarry:

    \begin{IEEEproof}
       \begin{IEEEeqnarray}{rCl+x*}
        x & = & y & \nonumber\IEEEQEDhere
       \end{IEEEeqnarray}
    \end{IEEEproof}

    While \IEEEQEDhereams is like amsthm's venerable \qedhere and is
    for use within the standard equation environment:

    \begin{IEEEproof}
     \begin{equation}
       x = y \nonumber\IEEEQEDhereams\quad
     \end{equation}
    \end{IEEEproof}

    Note that the qedhere style is normally not done with IEEE-related
    work so these are undocumented features of IEEEtran.cls.

    Thanks Mark D. Butala, Hennadiy Leontyev and Stefan M. Moser for
    suggesting this feature.



IEEEtrantools.sty is not needed and should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
2015/08/26 V1.5 (V1.8b of IEEEtran.cls) changes:

 1) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 2) Fix bug with IEEEeqnarray equation number foreground color
    under the color environment of Beamer class.
    Thanks to Joschi Brauchle for reporting this problem.

 3) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.



********************************** Files **********************************

README                - This file.

changelog.txt         - The revision history.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************


